Evaluating the Apperception Engine

The Apperception Engine is an unsupervised learning system. Given a sequence of sensory inputs, it constructs a symbolic causal theory that both explains the sensory sequence and also satisfies a set of unity conditions. The unity conditions insist that the constituents of the theory - objects, properties, and laws - must be integrated into a coherent whole. Once a theory has been constructed, it can be applied to predict future sensor readings, retrodict earlier readings, or impute missing readings. In this paper, we evaluate the Apperception Engine in a diverse variety of domains, including cellular automata, rhythms and simple nursery tunes, multi-modal binding problems, occlusion tasks, and sequence induction intelligence tests. In each domain, we test our engine's ability to predict future sensor values, retrodict earlier sensor values, and impute missing sensory data. The engine performs well in all these domains, significantly outperforming neural net baselines and state of the art inductive logic programming systems. These results are significant because neural nets typically struggle to solve the binding problem (where information from different modalities must somehow be combined together into different aspects of one unified object) and fail to solve occlusion tasks (in which objects are sometimes visible and sometimes obscured from view). We note in particular that in the sequence induction intelligence tests, our system achieved human-level performance. This is notable because our system is not a bespoke system designed specifically to solve intelligence tests, but a general-purpose system that was designed to make sense of any sensory sequence.

==> tex/discrete-complexity.tex <==
\subsection{Complexity}
\label{sec:complexity}

This section describes the complexity of Algorithm \ref{algo2}.

We assume basic concepts and standard terminology from complexity theory.
Let $P$ be the class of problems that can be solved in polynomial time by a deterministic Turing machine, 
$NP$ be the class of problems solved in polynomial time by a non-deterministic Turing machine, and $EXPTIME$ be the class of problems solved in time $2^{n^d}$ by a deterministic Turing machine.
Let $\Sigma_{i+1}^P = NP^{\Sigma_i^P}$ be the class of problems that can be solved in polynomial time by a non-deterministic Turing machine with a $\Sigma_i^P$ oracle.
If $\Pi$ is a Datalog program, and $A$ and $B$ are sets of ground atoms, then:
\begin{itemize}
\item
the \define{data complexity} is the complexity of testing whether $\Pi \cup A \models B$, as a function of $A$ and $B$, when $\Pi$ is fixed
\item
the \define{program complexity} (also known as ``expression complexity'') is the complexity of testing whether $\Pi \cup A \models B$, as a function of $\Pi$ and $B$, when $A$ is fixed
\end{itemize}
Datalog has polynomial time data complexity but exponential time program complexity: deciding whether a ground atom is in the least Herbrand model of a Datalog program is EXPTIME-complete. The reason for this complexity is because the number of ground instances of a clause is an exponential function of the number of variables in the clause.
Finding a solution to an ASP program is in NP \cite{ben1994propositional,dantsin2001complexity}, while finding an optimal solution to an ASP program with weak constraints is in $\Sigma^P_2$ \cite{brewka2003answer,gebser2011complex}.

Since deciding whether a non-disjunctive ASP program has a solution is in NP \cite{ben1994propositional,dantsin2001complexity}, our ASP encoding of Algorithm \ref{algo2} shows that finding a unified interpretation $\theta$ for a sequence given a template is in NP.
Since verifying whether a solution to an ASP program with preferences is indeed optimal is in $\Sigma^P_2$ \cite{brewka2003answer,gebser2011complex}, our ASP encoding shows that finding the lowest cost $\theta$ is in $\Sigma^P_2$.

However, the standard complexity results assume the ASP program has \emph{already been grounded into a set of propositional clauses}.
To really understand the space and time complexity of Algorithm \ref{algo2}, we need to examine how the set of ground atoms in the ASP encoding grows as a function of the parameters in the template $\chi = (\phi=(T, O, P, V), N_{\rightarrow}, N_{\fork}, N_B)$.

Observe that, since we restrict ourselves to unary and binary predicates, the number of ground and unground atoms is a small polynomial function of the type signature parameters\footnote{The actual numbers will be less than these bounds because type-checking rules out certain combinations.}:
\begin{eqnarray*}
|G_\phi| & \leq & |P| \cdot |O|^2 \\
|U_\phi| & \leq & |P| \cdot |V|^2
\end{eqnarray*}
But note that the number of substitutions $\Sigma_\phi$ that is compatible with the signature $\phi$ is an exponential function of the number of variables $V$:
\begin{eqnarray*}
|\Sigma_\phi| & \leq & |O|^{|V|}
\end{eqnarray*}
%Table \ref{table:complexity} shows the number of ground atoms for the most expensive predicates in the ASP encoding.
%Here, \verb|R| ranges over rules, \verb|VA| over unground atoms, \verb|Subs| over substitutions, \verb|Var| over variables, \verb|Obj| over objects, \verb|GA| over ground atoms, and \verb|T| over time-steps $1 .. t$.
%The predicates with the largest number of groundings are those that feature a variable of type \verb|Subs|.
%
%\begin{table}
%\centering
%\begin{tabular}{|l|l|}
%\hline
%{\bf Predicate} & {\bf Max \# ground atoms} \\
%\hline
%\verb|rule_body(R, VA)| & $|U_\phi| \cdot (N_{\rightarrow} + N_{\fork})$ \\
%\hline
%\verb|rule_head_static(R, VA)| & $|U_\phi| \cdot N_{\rightarrow}$ \\
%\hline
%\verb|rule_head_causes(R, VA)| & $|U_\phi| \cdot N_{\fork}$ \\
%\hline
%\verb|holds(GA, T)| & $|G_\phi| \cdot t$ \\
%\hline
%\verb|subs(Subs, Var, Obj)| & $|\Sigma_\phi| \cdot |V|$ \\
%\hline
%\verb|ground_atom(VA, GA, Subs)| & $|\Sigma_\phi| \cdot |U_\phi|$ \\
%\hline
%\verb|eval_atom(VA, Subs, T)| & $|\Sigma_\phi| \cdot |U_\phi| \cdot t$ \\
%\hline
%\verb|eval_body(R, Subs, T)| & $|\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot t$ \\
%\hline
%\end{tabular}
%\caption[The number of ground atoms in the ASP encoding]{The number of ground atoms in the ASP encoding of Algorithm \ref{algo2}.}
%\label{table:complexity}
%\end{table}
%
%From Table \ref{table:complexity}, we can see that the number of ground atoms is a linear function of the number of time-steps, a quadratic function of the number of objects, and an exponential function of the number of variables.

%
%In terms of the number of ground clauses, the most expensive rule in the ASP encoding is:
%\begin{Verbatim}[baselinestretch=0.9]
%holds(GA, T) :-
%    rule_arrow_head(R, VA),
%    eval_body(R, Subs, T),
%    ground_atom(VA, GA, Subs).
%\end{Verbatim}
%This rule generates $|\Sigma_\phi| \cdot |U_\phi| \cdot N_{\rightarrow} \cdot t$ ground instances, each containing 4 atoms.
%There is a similar number of ground clauses for the causal rules.
%
%The frame axiom is less expensive.
%\begin{Verbatim}[baselinestretch=0.9]
%holds(S, T+1) :-
%    holds(S, T),
%    is_time(T+1),
%    not -holds(S, T+1).
%\end{Verbatim}
%This generates $|G_\phi| \cdot t$ ground clauses. 
%There are only another $|G_\phi|$ ground clauses for the clause \verb|holds(A, 1) :- init(A).|
%
%Another clause that generates a large number of ground clauses is:
%\begin{Verbatim}[baselinestretch=0.9]
%eval_body(R, Subs, T) :-
%    is_rule(R),
%    is_subs(Subs),
%    is_time(T),
%    eval_atom(V, Subs, T) : rule_body(R, V).
%\end{Verbatim}
%This generates $|\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot t$ ground clauses, each of which contains $|U_\phi| + 4$ atoms.

Table \ref{table:num-ground-clauses} shows the number of ground clauses for the three most expensive clauses.
The total number of ground atoms for the three most expensive clauses is approximately $5 \cdot |\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot |U_\phi| \cdot t$.

\begin{table}
\centering
\begin{tabular}{|l|l|}
\hline
{\bf Predicate} & {\bf \# ground clauses} \\
\hline
\verb|holds| & $|\Sigma_\phi| \cdot |U_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot t + |G_\phi| \cdot (t+1)$ \\
\hline
\verb|eval_atom(VA, Subs, T)| & $|\Sigma_\phi| \cdot |U_\phi| \cdot t$ \\
\hline
\verb|eval_body(R, Subs, T)| & $|\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot t$ \\
\hline
\end{tabular}
\caption{The number of ground clauses in the ASP encoding of Algorithm \ref{algo2}.}
\label{table:num-ground-clauses}
\end{table}

%Figure \ref{fig:ground-atoms} shows how the number of ground atoms increases exponentially as a function of the number of variables.
%Here, we plot the number of ground atoms with predicate \verb|eval_atom| as a function of the number of variables, when interpreting \emph{Twinkle Twinkle Little Star} from the music domain. 
%
%\begin{figure}
%\centering
%\begin{tikzpicture}
%\begin{semilogyaxis}[xlabel=\# vars,ylabel=\# ground atoms]
%\addplot[
%    color=red,
%    mark=*,
%    ]
%    coordinates {
%    (2,90)(3,1200)(4,2040)(5,6480)(6,69120)(7,92160)(8,293760)
%    };
%\end{semilogyaxis}
%\end{tikzpicture}
%\caption{How \# ground atoms grows (log-scale) as we increase \# vars}
%\label{fig:ground-atoms}
%\end{figure}




\begin{table}
\begin{center}
\begin{tabular}{|p{6.0cm}|r|r|}
\hline
{\bf Clause} & {\bf \# ground clauses} & {\bf \# atoms}\\
\hline
\begin{lstlisting} 
holds(GA, T) :-
    rule_head_static(R, VA),
    eval_body(R, Subs, T),
    ground_atom(VA, GA, Subs).\end{lstlisting}&
$|\Sigma_\phi| \cdot |U_\phi| \cdot N_{\rightarrow} \cdot t$
&
$4$ \\
\hline
\begin{lstlisting}
holds(GA, T+1) :-
    rule_head_causes(R, VA),
    eval_body(R, Subs, T),
    ground_atom(VA, GA, Subs).\end{lstlisting}&
$|\Sigma_\phi| \cdot |U_\phi| \cdot N_{\fork} \cdot t$
&
$4$ \\
\hline
%\begin{lstlisting}
%holds(S, T+1) :-
%    holds(S, T),
%    is_time(T+1),
%    not -holds(S, T+1).\end{lstlisting}&
%$|G_\phi| \cdot t$
%&
%$4$ \\
%\hline
\begin{lstlisting}
eval_body(R, Subs, T) :-
    is_rule(R),
    is_subs(Subs),
    is_time(T),
    eval_atom(V, Subs, T) : rule_body(R, V).\end{lstlisting}&
$|\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot t$
&
$|U_\phi| + 4$ \\
\hline
%\begin{lstlisting}
%0 { rule_body(R, VA) : is_unground_atom(VA) } k_max_body :- is_rule(R).\end{lstlisting}&
%$N_\rightarrow + N_{\fork}$
%&
%$|U_\phi|$ \\
%\hline
\end{tabular} 
\caption[The number of ground clauses in the ASP encoding]{The number of ground clauses in the ASP encoding of Algorithm \ref{algo2}.}
\label{table:num-ground-clauses}
\end{center}
\end{table}

\subsection{Optimization}
\label{sec:optimization}

Because of the combinatorial complexity of the apperception task, 
we had to introduce a number of optimizations to get reasonable performance on even the simplest of domains.

\subsubsection{Reducing grounding with type checking}
\label{sec:type-checking}

We use the type signature $\phi$ to dramatically restrict the set of ground atoms ($G_\phi$), the unground atoms ($U_\phi$), the substitutions ($\Sigma_\phi$), and rules $R_\phi$. 
Type-checking has been shown to drastically reduce the search space in program synthesis tasks \cite{typing-morel}.

\subsubsection{Symmetry breaking}
\label{sec:symmetry-breaking}

We use symmetry breaking to remove candidates that are equivalent.
For example, the following two rules are equivalent up to variable renaming:
\begin{eqnarray*}
p(X, Y) & \rightarrow & q(X) \\
p(Y, X) & \rightarrow & q(Y)
\end{eqnarray*}
We prune the second rule by using a strict partial order on variables:
$X < Y$ if $X$ and $Y$ are of the same type (if $\kappa_V(X) = \kappa_V(Y)$) and $X$ is lexicographically before $Y$.
Now we prune rules where there is a variable $X$ in the body $B$, where $Y < X$ and it is not the case that either:
\begin{itemize}
\item
there is an atom $p(Y)$ in $B$, or:
\item
there is an atom $p(Y, X)$ in $B$
\end{itemize}
The second form of symmetry breaking is to prune collections of rules that are equivalent up to reordering.
Because we represent rules using rule-identifiers, there are multiple rule-sets that are equivalent but represented distinctly.
For example, the sets $R_1$ and $R_2$ are obviously equivalent:
\begin{eqnarray*}
R_1 = \begin{cases}
r_1 : p(X) \rightarrow q(X) \\
r_2 : q(X) \rightarrow r(X)
\end{cases} \\
R_2 = \begin{cases}
r_1 : q(X) \rightarrow r(X) \\
r_2 : p(X) \rightarrow q(X)
\end{cases}
\end{eqnarray*}

We define a strict total ordering $<$ on unground atoms in $U_\phi$, and use this to prune duplicates.
We disallow any rule-set that contains two rules $r_i : B \rightarrow \alpha$ and $r_j : B' \rightarrow \alpha'$ where $i < j$ and there exists an atom $\beta' \in B'$ that is $<$ every atom $\beta \in B$.
Assuming that $p(X) < q(X) < r(X)$, this rules out $R_2$ in the example above.

\subsubsection{Adding redundant constraints}
\label{sec:redundant-constraints}

ASP programs can be significantly optimized by adding redundant constraints (constraints that are provably entailed by the other clauses in the program) \cite{gebser2012answer}.
We speeded up solving time (by about 30\%) by adding the following redundant constraints:
\begin{Verbatim}[baselinestretch=0.9]
:-  init(A),
    init(B),
    incompossible(A, B).

:-  rule_body(R, A),
    rule_body(R, B),
    incompossible_var_atoms(A, B).    

:-  rule_body(R, A),
    rule_head_static(R, A).

:-  rule_body(R, A),
    rule_head_causes(R, A).

:-  rule_body(R, A),
    rule_head_static(R, B),
    incompossible_var_atoms(A, B).    

:-  rule_body(R, A),
    rule_head_causes(R, B),
    incompossible_var_atoms(A, B).    
\end{Verbatim}     

%\subsubsection{Replacing the meta-interpreter of constraints with compiled clauses}
%\label{sec:compiling-eval}
%
%In an earlier implementation, the $\mathit{xor}$ and $\exists !$ constraints were evaluated using a meta-interpreter (as the rules are).
%We made a significant optimization (approximately 10x speed-up) by replacing this part of the meta-interpreter with compiled clauses.
%Here, we used the same approach as ASPAL \cite{corapi2012inductive} and ILASP \cite{law2014inductive} to compile the constraint clauses directly into ASP.
%Removing the overhead of the interpreter gave us a large speedup here.
%But note that we did not replace the $\tau(\theta)$ interpreter with a set of compiled clauses.
%The reason it is worth compiling the constraint evaluator -- but it is not worth compiling the update rules -- is because of the relatively small number of possible constraints. 
%The number of possible update rules grows quickly with the number of unground atoms, so compiling each possible update rule into an ASP clause is prohibitively expensive. See Section \ref{sec:ilasp} for an empirical evaluation comparing the grounding sizes of the programs when meta-interpreting the update rules versus compiling the update rules.



==> tex/discrete-conclusion.tex <==


\section{Discussion}
\label{sec:conclusion}

This chapter is an attempt to answer a key question of unsupervised learning: what does it mean to ``make sense'' of a (discretised) sensory sequence? 
Our answer is broadly Kantian \cite{chalmers1992high}: making sense means positing a collection of objects that persist over time, with attributes that change over time, according to intelligible laws.
As well as providing a precise formalization of this task, we also provide a concrete implementation of a system that is able to make sense of the sensory stream.
We have tested the \sys{} in a variety of domains;
in each domain, we tested its ability to predict future values, retrodict previous values, and impute missing intermediate values. 
Our system achieves good results across the board.

Of particular note is that it is able to achieve human performance on challenging sequence induction IQ tasks.
We stress, once more, that the system was not hard-coded to solve these tasks.
Rather, it is a general \emph{domain-independent} sense-making system that is able to apply its general architecture to the particular problem of Seek Whence induction tasks, and is able to solve these problems ``out of the box'' without human hand-engineered help.
We also stress, again, that the system did not learn to solve these sequence induction tasks by being presented with hundreds of training examples\footnote{
Raven's progressive matrices \cite{carpenter1990one}  are spatial reasoning tasks requiring inductive reasoning. 
Barrett et al \cite{barrett2018measuring} train a neural network to learn to solve Raven's progressive matrices, but their method requires millions of training examples.}. 
Indeed, the system had never seen a \emph{single} such task before.
Instead, it applied its general sense-making urge to each individual task, \emph{de novo}.
We also stress that the interpretations produced are human readable and can be used to provide explanations and justifications of the decisions taken:
when the \sys{} produces an interpretation, we can not only see what it predicts will happen next, but we can also understand \emph{why} it thinks this is the right continuation. 
We believe these results are highly suggestive, and shows that a sense-making component such as this will be a key aspect of any general intelligence.
%We do not claim, of course, that any such sense-making machine must have the same precise architecture as that described in Section \ref{sec:system}. But we \emph{do} claim that it must satisfy the conditions of sense-making of Definition \ref{def:apperception-task}. 

Our architecture, an unsupervised program synthesis system, is a purely symbolic system, and 
as such, it inherits two key advantages of ILP systems \cite{evans2018learning}.
First, the interpretations produced are \emph{interpretable}. 
Because the output is symbolic, it can be read and verified by a human\footnote{Large machine-generated programs are not always easy to understand. But machine-generated symbolic programs are certainly easier to understand than the weights of a neural network. See Muggleton et al \cite{muggleton2018ultra} for an extensive discussion. }.
Second, it is very \emph{data-efficient}.
Because of the language bias of the \logic{} language, and the strong inductive bias provided by the Kantian unity conditions, the system is able to make sense of extremely short sequences of sensory data, without having seen any others.
%The reason for this data-efficiency is the language bias preferring short programs over longer ones: a short general program will be preferred to a larger program consisting of many special-case ad-hoc rules that happen to cover the input sequence.
%A third key advantage of symbolic program synthesis methods is that they support continual learning as solutions learned in one task can be reused in the next to reduce the search-space\cite{lin2014bias}.

However, the system in its current form has some clear limitations.
First, it does not currently handle noise in the sensory input.
All sensory information is assumed to be significant, and the system will strive to find an explanation of \emph{every} sensor reading.
There is no room for the idea that some sensor readings are inaccurate.

Second, the sensory input must be discretized before it can be passed to the system.
We assume some prior system has already discretized the continuous sensory values by grouping them into classes.

The first limitation is addressed in Section \ref{sec:noise}, and the second limitation is addressed in Chapter \ref{chapter:making-sense-raw}.



==> tex/discrete-house.tex <==
\section{Experiment 2: the house}
\label{sec:house}

In the \emph{Second Analogy}, Kant describes the following example:
\begin{quote}
The apprehension of the manifold of appearance is always successive. The representations of the parts succeed one another. Whether they also succeed in the object is a second point for reflection, which is not contained in the first... Thus, e.g., the apprehension of the manifold in the appearance of a house that stands before me is successive. Now the question is whether the manifold of this house itself is also successive, which certainly no one will concede. [A189/B234ff] 
\end{quote}
Here, Kant asks us to imagine an agent surveying a large house from close range. Its visual field cannot take in the whole house in one glance, so its focus moves from one part of the house to another.
Its sequence of visual impressions is successive, but there is a further question whether a pair of (subjectively) successive visual impressions represents the house at a single moment of objective time, or at two successive moments of objective time.

In the B edition of the \emph{Transcendental Deduction}, Kant contrasts the example of the house with another example: an agent watching water slowly freeze:
\begin{quote}
Thus if, e.g., I make the empirical intuition of a house into perception through apprehension of its manifold, my ground is the necessary unity of space and of outer sensible intuition in general, and I as it were draw its shape in agreement with this synthetic unity of the manifold in space...
If (in another example) I perceive the freezing of water, I apprehend two states (of fluidity and solidity) as ones standing in a relation of time to each other.
[B162]
\end{quote}
Kant asks us to compare and contrast the two cases of subjective succession. 
In the first case, the subjective succession represents an \emph{objective simultaneity}: the perceived state of the top of the house is simultaneous with the perceived state of the bottom of the house, even if the subjective impressions are successive. 
In the second case, by contrast, the subjective succession represents an \emph{objective succession}: the water's transition from liquid to solid is a fact about the world, not just about my mental states. 
Kant characterises the difference between the two cases in terms of modality: in the case of the house, I could have received the impressions in a different order: I could have seen the bottom of the house before the top. But in the case of the water freezing, I could not have seen the solid state before the liquid state.\footnote{See \cite[p.358]{longuenesse1998kant}.}

We gave the \sys{} a simplified version of Kant's example (see Figure \ref{fig:house-1}).
In our experiment, there is a pixel image that is too large for the agent to survey in one glance. 
The agent's sensors are only able to take in a small window of the image at any moment, and the agent must move the sensory window around to survey the whole image. 
Just as in Kant's case, where we cannot take in the whole of the house in one glance, here the agent cannot take in the whole of the pixel image at one glance,  and must reconstruct it from the succession of fragments. 

Note that in this experiment, the actions are exogenous and do not need to be explained by the \sys{}.
What does need to be explained is the changing sensor information.

When we give the sequence of Figure \ref{fig:house-1} to the \sys{}, it is able to reconstruct the complete picture from the sequence of incomplete partial perceptions.
The best theory it finds is $\theta = (\phi, I, R, C)$ where:
\begin{eqnarray*}
I & = & \bigsetbegin{} 
\begin{tabular}{llll}
$\mathit{off}(w_{1,2})$ &
$\mathit{off}(w_{1,3})$ &
$\mathit{off}(w_{2,3})$ &
$\mathit{off}(w_{3,2})$ \\
$\mathit{off}(w_{4,2})$ &
$\mathit{off}(w_{4,3})$ &
$\mathit{on}(w_{1,1})$ &
$\mathit{on}(w_{1,4})$ \\
$\mathit{on}(w_{2,1})$ &
$\mathit{on}(w_{2,2})$ &
$\mathit{on}(w_{2,4})$ &
$\mathit{on}(w_{3,1})$ \\
$\mathit{on}(w_{3,3})$ &
$\mathit{on}(w_{3,4})$ &
$\mathit{on}(w_{4,1})$ &
$\mathit{on}(w_{4,4})$ \\
$\mathit{in}(v_{1,1}, w_{1,4})$ &
$\mathit{in}(v_{1,2}, w_{1,3})$ &
$\mathit{in}(v_{2,1}, w_{2,4})$ &
$\mathit{in}(v_{2,2}, w_{2,3})$
\end{tabular}
\bigsetend{} \\
R & = & \bigsetbegin{} 
\mathit{off}(W) \wedge \mathit{in}(V, W) \wedge \mathit{zero}(N) \rightarrow \mathit{intensity}(V, N) \\
\mathit{on}(W) \wedge \mathit{in}(V, W) \wedge \mathit{one}(N) \rightarrow \mathit{intensity}(V, N) \\
\mathit{right}(M) \wedge r(W, W_2) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2) \\
\mathit{left}(M) \wedge r(W_2, W) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2) \\
\mathit{up}(M) \wedge b(W, W_2) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2) \\
\mathit{down}(M) \wedge b(W_2, W) \wedge \mathit{in}(V, W) \fork \mathit{in}(V, W_2)
\bigsetend{} \\
C & = & \bigsetbegin{}
\forall C{:}\mathit{cell}, \mathit{on}(X) \oplus \mathit{off}(X) \\
\forall V{:}\mathit{sensor}, \exists ! C{:}\mathit{cell}, \mathit{in}(V, C) \\
\forall V{:}\mathit{sensor}, \exists ! N{:}\mathit{number}, \mathit{intensity}(C, N)
\bigsetend{}
\end{eqnarray*}
Here, the initial conditions $I$ specify the on/off values of the sixteen pixels $\{w_{i,j} \mid i \in \{1..4\}, j \in \{1..4\}\}$, and the initial placements of the four sensors $\{v_{i,j} \mid i \in \{1,2\}, j \in \{1,2\}\}$.
Note that the on/off values of the  pixels do not change over time. 
The 2D spatial relations between the cells $w_{i,j}$ are represented by the $r$ and $b$ relations. E.g. $r(w_{1,1}, w_{2,1})$, $b(w_{1,1}, w_{1,2})$. The spatial relations using $r$ and $b$ are provided as background knowledge.

The first two rules state that if a sensor is attached to a cell, and that cell is on (respectively off), then the intensity of the sensory is 1 (respectively 0).
The other rules describe how the sensors move as the actions are performed.
Note that the image reconstructed by the \sys{} is a mirror image of the original image used to generate the sensory data.
Figure \ref{fig:house-2}(b) shows the sequence as reconstructed by the \sys{}.
In this interpretation, the original image has been flipped vertically, and the actions ``up'' and ``down'' have been interpreted as ``down'' and ``up'' respectively.


\begin{figure}
\centering
\includegraphics[scale=0.4]{figs/kant/house-full.pdf}
\caption[The sensory sequence for the ``house'' example]{For each of the sixteen time-steps, we show the $4 \times 4$ pixel grid and the positions of the sensors (as a red square), the action performed, and the values of the four sensors. }
\label{fig:house-1}
\end{figure}


\begin{figure}
\centering
\begin{minipage}{13 cm}
  \subfloat[]{%
    \makebox[\textwidth][c]{\includegraphics[scale=0.4]{figs/kant/house1.pdf}}
  }
  \\
  \subfloat[]{%
    \makebox[\textwidth][c]{\includegraphics[scale=0.4]{figs/kant/house2.pdf}}
  }  
\caption[Comparing the ground truth with the engine's reconstruction]{The top row (a) shows the ground truth used to generate the sensory data, while the bottom row (b) shows the reconstruction made by the \sys{}. Note that the reconstruction is a mirror image of the ground truth, flipped vertically, in which ``up'' is interpreted as down, and ``down'' is interpreted as up. }
\label{fig:house-2}
\end{minipage}
\end{figure}

Thus, the \sys{} is able to make sense of Kant's famous ``house'' example [B162]:
the engine posits a two-dimensional array of pixels and interprets the sensors as moving across the array.
Although the sensory readings are successive, the engine posits an \emph{objective simultaneity} to explain the subjective succession of sensor readings. % For example, the pixel at (1,1) being on is simultaneous with the pixel at (1,2) being off.



==> tex/discrete-interpreter.tex <==
\subsection{The ASP encoding}
\label{sec:computational-details}

Our \logic{} interpreter is written in ASP.
All elements of \logic{}, including variables, are represented by ASP constants.
A variable $X$ is represented by a constant \verb|var_x|, and a predicate $p$ is represented by a constant \verb|c_p|.
Elements of the target language are \emph{reified} in ASP, so an unground atom $p(X)$ of \logic{} is represented by a term \verb|s(c_p, var_x)|, and 
a rule is represented by a set of ground atoms for the body, and a single ground atom for the head.
For example, the static rule $p(X) \wedge q(X, Y) \rightarrow r(Y)$ is represented as:
\begin{Verbatim}[baselinestretch=0.9]
rule_body(r1, s(c_p, var_x)). 
rule_body(r1, s2(c_q, var_x, var_y)). 
rule_head_static(r1, s(c_r, var_y)). 
\end{Verbatim}
The causal rule $\mathit{on}(X) \fork \mathit{off}(X)$ is represented as:
\begin{Verbatim}[baselinestretch=0.9]
rule_body(r2, s(c_on, var_x)). 
rule_head_causes(r2, s(c_off, var_x)). 
\end{Verbatim}
Given a type signature $\phi$, we construct ASP terms that represent every well-typed unground atom in $U_\phi$, and wrap these terms in the \verb|is_var_atom| predicate. 
For example, to represent that $r(C, C_2)$ is a well-typed unground atom, we write \verb|is_var_atom(atom(c_r, var_c, var_c2))|.
Similarly, we construct ASP terms that represent every well-typed ground atom in $G_\phi$ using the \verb|is_ground_atom| predicate.

%We also construct ASP atoms that represent every substitution in $\Sigma_\phi$. For each substitution $\sigma$ and each $X/k $ in $\sigma$, we add an atom of the form $\mathsf{subs}(\sigma, X, k)$. For example, we represent $\sigma_{17} = \{X/a, Y/b\}$ as:
%\begin{Verbatim}[baselinestretch=0.9]
%subs(subs_17, var_x, obj_a).
%subs(subs_17, var_y, obj_b).
%\end{Verbatim}
%To represent that the result of applying substitution $\sigma$ to unground atom $\alpha$ is ground atom $\alpha'$, we use the \verb|ground_atom| predicate:
%\begin{Verbatim}[baselinestretch=0.9]
%ground_atom(s(C, V), s(C, Obj), Subs) :-
%    is_var_fluent(s(C, V)),
%    subs(Subs, V, Obj).
%
%ground_atom(s2(C, V, V2), s2(C, Obj, Obj2), Subs) :-
%    is_var_fluent(s2(C, V, V2)),
%    subs(Subs, V, Obj),
%    subs(Subs, V2, Obj2).
%\end{Verbatim}

The initial conditions $I \subseteq G_\phi$ are represented by the \verb|init| predicate. 
For example, to represent that $I = \{p(a), r(b, c)\}$, we write:
\begin{Verbatim}[baselinestretch=0.9]
init(s(c_p, c_a)).
init(s2(c_r, c_b, c_c)).
\end{Verbatim}

Our meta-interpreter $\pi_\tau$ implements $\tau : \Theta \rightarrow (2^\mathcal{G})^*$ from Definition \ref{def:trace}. We use \verb|holds(a, t)| to represent that atom \verb|a| is true at time \verb|t| (i.e. $a \in S_t$ where $\tau(\theta) = (S_1, S_2, ..., S_t, ...)$).
\begin{Verbatim}[baselinestretch=0.9]
% initial conditions
holds(A, T) :-
    init(A),
    init_time(T).

% update for static rules
holds(GA, T) :-
    rule_arrow_head(R, VA),
    eval_body(R, Subs, T),
    ground_atom(VA, GA, Subs).

% update for causal rules
holds(GC, T+1) :-     
    rule_head_causes(R, VC),
    eval_body(R, Subs, T),
    ground_atom(VC, GC, Subs),
    is_time(T+1).

% frame axiom
holds(S, T+1) :-
    holds(S, T),
    is_time(T+1),
    not -holds(S, T+1).
\end{Verbatim}    
Since $\tau(\theta)$ is an infinite sequence $(A_1, A_2, ...)$, we cannot compute the whole of it.
Instead, we only compute the sequence up to the max time of the original sensory sequence $S$.

Note that the frame axiom uses negation as failure and strong negation \cite{baral1994logic} to check that some other incompatible atom has not already been added. 
Thus, the frame axiom is not restrictive and can be overridden as needed by the causal rules, to handle predicates that are not inertial.

The conditions of unity described in Section \ref{sec:unity-conditions} are represented directly as ASP constraints in $\pi_u$.
For example, spatial unity is encoded as:
\begin{Verbatim}[baselinestretch=0.9]
:-  spatial_unity_counterexample(X, Y, T).
\end{Verbatim}
Here, there is a counterexample to spatial unity at time \verb|T| if objects \verb|X| and \verb|Y| are not \verb|related|:
\begin{Verbatim}[baselinestretch=0.9]
spatial_unity_counterexample(X, Y, T) :-
    is_object(X),
    is_object(Y),
    is_time(T),
    not related(X, Y, T).
\end{Verbatim}
Here, \verb|related| is the reflexive symmetric transitive closure of the relation holding between \verb|X| and \verb|Y| if there is some relation \verb|R| connecting them.
Note that \verb|related| can quantify over relations because the \logic{} atoms and predicates have been reified into terms:
\begin{Verbatim}[baselinestretch=0.9]
related(X, Y, T) :-
    holds(s2(R, X, Y), T).

related(X, X, T) :-
    is_object(X),
    is_time(T).
    
related(X, Y, T) :- related(Y, X, T).

related(X, Y, T) :-
    related(X, Z, T),
    related(Z, Y, T).
\end{Verbatim}

When constructing a theory $\theta = (\phi, I, R, C)$, the solver needs to choose which ground atoms to use as initial conditions in $I$, which static and causal rules to include in $R$, and which xor or uniqueness conditions to use as conditions in $C$.

To allow the solver to choose what to include in $I$, we add the ASP choice rule to $\pi_I$:
\begin{Verbatim}[baselinestretch=0.9]
{ init(A) } :- is_ground_atom(A).
\end{Verbatim}

To allow the solver to choose which rules to include in $R$, we add the following clauses to $\pi_R$:
\begin{Verbatim}[baselinestretch=0.9]
0 { rule_body(R, VA) : is_var_atom(VA) } k_max_body :- is_rule(R).
1 { rule_head_static(R, VA) : is_var_atom(VA) } 1 :- is_static_rule(R).
1 { rule_head_causes(R, VA) : is_var_atom(VA) } 1 :- is_causes_rule(R).
\end{Verbatim}
Here, \verb|k_max_body| is the $N_B$ parameter of the template that specifies the max number of body atoms in any rule.
The number of rules satisfying \verb|is_static_rule| and \verb|is_causes_rule| is determined by the parameters $N_{\fork}$ and $N_\rightarrow$ in the template (see Definition \ref{def:template}). 

The ASP program $\pi_m$ minimizes the cost of the theory $\theta$ (see Definition \ref{def:theory-cost}) by using weak constraints \cite{calimeri2012asp}:
\begin{eqnarray*}
& & \asp{:\sim  rule\_body(R, A). \; [1 @ 1, R, A]} \\
& & \asp{:\sim  rule\_arrow\_head(R, A). \; [1 @ 1, R, A]} \\
& & \asp{:\sim  rule\_causes\_head(R, A). \; [1 @ 1, R, A]} \\
& & \asp{:\sim  init(A). \; [1 @ 1, A]} 
\end{eqnarray*}


%Constraints in $C$ are represented directly as ASP constraints.
%For example, if $k_1$ is the constraint $\forall X{:}\mathit{cell}, \mathit{on}(X) \oplus \mathit{off}(X)$, then $k_1$ is represented as:
%\begin{Verbatim}[baselinestretch=0.9]
%:-  holds(s(c_on, X), T),
%    holds(s(c_off, X), T),
%    use_constraint(k_1).
%    
%:-  isa(X, t_cell),
%    is_time(T),
%    not holds(s(c_on, X), T),
%    not holds(s(c_off, X), T),
%    use_constraint(k_1).
%    
%incompossible(s(c_on, X), s(c_off, X)) :-
%    isa(X, t_cell),
%    use_constraint(k_1).    
%\end{Verbatim}
%Here, the flag \verb|use_constraint(k_1)| is used to check whether or not we wish to include this particular constraint in $C$. 
%The solver chooses which particular constraints to use, just as it gets to choose the initial atoms and the update rules.
%For example, if there are four unary predicates $p_1, ..., p_4$, there are various possible sets of constraints that each satisfy conceptual unity:
%\begin{eqnarray*}
%\set{p_1(X) \oplus p_2(X), p_3(X) \oplus p_4(X)} \\
%\set{p_1(X) \oplus p_3(X), p_2(X) \oplus p_4(X)} \\
%\set{p_1(X) \oplus p_4(X), p_2(X) \oplus p_3(X)} \\
%\set{p_1(X) \oplus p_2(X) \oplus p_3(X) \oplus p_4(X)}
%\end{eqnarray*}
%
%To allow the solver to choose which constraints to include in $C$, we generate all possible sets of constraints and add a cardinality constraint that exactly one such set is active for each type.
%For example, if there are four unary predicates $p_1(t), ... p_4(t)$ of type $t$, then there are various ways of collecting them into xor groups:
%\begin{eqnarray*}
%\set{p_1(X) \oplus p_2(X), p_3(X) \oplus p_4(X)} \\
%\set{p_1(X) \oplus p_3(X), p_2(X) \oplus p_4(X)} \\
%\set{p_1(X) \oplus p_4(X), p_2(X) \oplus p_3(X)} \\
%\set{p_1(X) \oplus p_2(X) \oplus p_3(X) \oplus p_4(X)}
%\end{eqnarray*}
%We remove sets that are equivalent up to renaming, so are left with:
%\begin{eqnarray*}
%\set{p_1(X) \oplus p_2(X), p_3(X) \oplus p_4(X)} \\
%\set{p_1(X) \oplus p_2(X) \oplus p_3(X) \oplus p_4(X)}
%\end{eqnarray*}
%Let us call these two xor sets $k_1$ and $k_2$.
%We use flags \verb|use_constraint(k_1)| and \verb|use_constraint(k_2)| to indicate which xor set to use, and add the cardinality constraint: 
%\begin{Verbatim}[baselinestretch=0.9]
%1 { use_constraint(k_1), use_constraint(k_2) } 1.
%\end{Verbatim}



==> tex/discrete-noise.tex <==


\section{Noisy apperception}
\label{sec:noise}


So far, we have assumed that our sensor readings are entirely noise-free:
some of the sensory readings may be missing, but none of the readings are inaccurate.

If we give the \sys{} a sensory sequence with mislabeled data, it will struggle to provide a theoretical explanation of the mislabeled input.
Consider, for example, $S_{1:20}$:
\begin{eqnarray*}
\begin{tabular}{lllll}
$S_1 = \set{p(a)}$  & $S_2 = \set{p(a)}$ & $S_3 = \set{ \mathbf{q(a)}}$ & $S_4 = \set{p(a)}$  & $S_5 = \set{p(a)}$ \\
 $S_6 = \set{ p(a)}$ & $S_7 = \set{p(a)}$  & $S_8 = \set{p(a)}$ & $S_9 = \set{ p(a)}$ & $S_{10} = \set{p(a)}$  \\
$S_{11} = \set{p(a)}$ & $S_{12}= \set{ p(a)}$ & $S_{13} = \set{p(a)}$  & $S_{14} = \set{p(a)}$ & $S_{15} = \set{ p(a)}$ \\
$S_{16} = \set{p(a)}$  & $S_{17} = \set{p(a)}$ & $S_{18} = \set{ p(a)}$ &$S_{19} = \set{p(a)}$ & $S_{20} = \set{p(a)}$
\end{tabular}
\end{eqnarray*}
Here, $S_3 = \set{ \mathbf{q(a)}}$ is an outlier in the otherwise tediously predictable sequence.

If we give sequences such as this to the \sys{}, it attempts to make sense of \emph{all} the input, including the anomalies. 
In this case, it finds the following baroque explanation:
\begin{eqnarray*}
\begin{tabular}{lll}
$I = \bigsetbegin{}
p(a) \\
c_1(a)
\bigsetend{}$ &
$R = \bigsetbegin{}
q(X) \rightarrow c_3(X) \\
c_3(X) \fork p(X) \\
c_1(X) \fork c_2(X) \\
c_2(X) \fork q(X)
\bigsetend{}$ &
$C' = \bigsetbegin{}
\forall X {:}s, \; p(X) \oplus q(X) \\
\forall X {:}s, \; c_1(X) \oplus c_2(X) \oplus c_3(X)
\bigsetend{}$
\end{tabular}
\end{eqnarray*}
Here, the \sys{} has introduced three new invented predicates $c_1, c_2, c_3$ in order to count how many $p$'s it has seen, so that it knows when to switch to $q$.
If we move the anomalous entry $q(a)$ later in the sequence, or add further anomalies, the engine is forced to construct increasingly complex theories.
This is clearly unsatisfactory.

In order to handle noisy mislabeled data, we shall relax our insistence that the sequence $S_{1:T}$ is \emph{entirely} covered by the trace of the theory $\theta$.
Instead of insisting that $S \sqsubseteq \tau(\theta)$, we shall minimise the number of discrepancies between each $S_i$ and $\tau(\theta)_i$, for $i = 1 .. T$.

We want to find the most probable theory $\theta$ given our noisy input sequence $S_{1:T}$:
\begin{eqnarray}
\label{eqn:noisy-1}
\argmax_{\theta} \; p\left(\theta \mid S_{1:T}\right)
\end{eqnarray}
By Bayes' rule, this is equivalent to
\begin{eqnarray}
\label{eqn:noisy-2}
\argmax_{\theta} \; \frac{p(\theta) \cdot p\left(S_{1:T} \mid \theta \right)}{p(S_{1:T})}
\end{eqnarray}
Since the denominator does not depend on $\theta$, this is equivalent to:
\begin{eqnarray}
\label{eqn:noisy-3}
\argmax_{\theta} \; p(\theta) \cdot p\left(S_{1:T} \mid \theta \right)
\end{eqnarray}
Since the probability of the sequence $S_{1:T}$ given the theory is just the product of the probabilities of each state given the theory, the above is equivalent to:
\begin{eqnarray}
\label{eqn:noisy-4}
\argmax_{\theta} \; p(\theta) \cdot \prod_{i=1}^T p\left(S_i \mid \theta \right)
\end{eqnarray}
Now each $S_i$ depends only on $\tau(\theta)_i$, the trace of $\theta$ at time step $i$.
Thus we can rewrite to:
\begin{eqnarray}
\label{eqn:noisy-5}
\argmax_{\theta} \; p(\theta) \cdot \prod_{i=1}^T p\left(S_i \mid \tau(\theta)_i \right)
\end{eqnarray}
Let the probability of $\theta$ be $2^{-\mathit{len}(\theta)}$.
Let\footnote{If we want to weight unexplained ground atoms differently from unground atoms of the theory, we could add a $\beta$ parameter and use the more general formula $p\left(S_i \mid \tau(\theta)_i \right) = 2^{-\beta \cdot |S_i - \tau(\theta)_i|}$.} the probability of  $S_i$ given $\tau(\theta)_i$ be $p\left(S_i \mid \tau(\theta)_i \right) = 2^{-|S_i - \tau(\theta)_i|}$.
Then we can rewrite to:
\begin{eqnarray}
\label{eqn:noisy-6}
\argmax_{\theta} \; 2^{-\mathit{len}(\theta)} \cdot \prod_{i=1}^T 2^{-|S_i - \tau(\theta)_i|}
\end{eqnarray}
Since $\mathit{log}_2$ is monotonic, we can take logs and rewrite to:
\begin{eqnarray}
\label{eqn:noisy-7}
\argmax_{\theta} \;  -\mathit{len}(\theta) + \sum_{i=1}^T -|S_i - \tau(\theta)_i|
\end{eqnarray}
Thus, we define the \define{$\mathit{cost}_\mathit{noise}$} of the theory to be:
\begin{eqnarray}
\label{eqn:noisy-8}
\mathit{cost}_\mathit{noise} = \mathit{len}(\theta) + \sum_{i=1}^T |S_i - \tau(\theta)_i|
\end{eqnarray}
and search for the theory with lowest cost.

\begin{example}
Consider, for example, the following sequence $S_{1:10}$:
\begin{eqnarray*}
\begin{tabular}{lllll}
$S_1 = \set{}$  & $S_2 = \set{ \mathit{off}(a), \mathit{on}(b)}$ & $S_3 = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S_4 = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S_5 = \set{ \mathit{on}(b)}$ \\
$S_6 = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S_7 = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S_8 = \set{ \mathit{off}(a), \mathit{on}(b)}$ & $S_9 = \set{ \mathit{on}(a)}$ & $S_{10} = \set{ }$
\end{tabular}
\end{eqnarray*}
Because the sequence is so short, the lowest $\mathit{cost}_\mathit{noise}$ theory is:
\begin{eqnarray*}
\begin{tabular}{lll}
$I = \bigsetbegin{}
\bigsetend{}$ &
$R = \bigsetbegin{}
\bigsetend{}$ &
$C' = \bigsetbegin{}
\forall X {:}s, \; \mathit{on}(X) \oplus \mathit{off}(X)
\bigsetend{}$
\end{tabular}
\end{eqnarray*}
This degenerate empty theory has cost 14 (the number of atoms in $S$) which is shorter than any ``proper'' explanation that captures the regularities.
But as the sequence gets longer, the advantage of a ``proper'' explanation over a degenerate solution becomes more and more apparent.
Consider, for example, the following extension $S'_{1:30}$:
\begin{eqnarray*}
\begin{tabular}{lllll}
$S'_1 = \set{}$  & $S'_2 = \set{ \mathit{off}(a), \mathit{on}(b)}$ & $S'_3 = \set{ \mathit{on}(a),  \mathit{off}(b)}$ &
$S'_4 = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_5 = \set{ \mathit{on}(b)}$ \\
$S'_6 = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S'_7 = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_8 = \set{ \mathit{off}(a), \mathit{on}(b)}$ & $S'_9 = \set{ \mathit{on}(a)}$ & $S'_{10} = \set{ }$ \\ 
$S'_{11}= \set{ \mathit{off}(a), \mathit{on}(b)}$ &  $S'_{12} = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S'_{13} = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_{14}= \set{ \mathit{off}(a), \mathit{on}(b)}$ &  $S'_{15} = \set{ \mathit{on}(a),  \mathit{off}(b)}$ \\
$S'_{16} = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_{17}= \set{ \mathit{off}(a), \mathit{on}(b)}$ &  $S'_{18} = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S'_{19} = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_{20}= \set{ \mathit{off}(a), \mathit{on}(b)}$ \\  
$S'_{21} = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S'_{22} = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_{23}= \set{ \mathit{off}(a), \mathit{on}(b)}$ &  $S'_{24} = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S'_{25} = \set{ \mathit{on}(a), \mathit{on}(b)}$ \\
$S'_{26}= \set{ \mathit{off}(a), \mathit{on}(b)}$ &  $S'_{27} = \set{ \mathit{on}(a),  \mathit{off}(b)}$ & $S'_{28} = \set{ \mathit{on}(a), \mathit{on}(b)}$ & $S'_{29}= \set{ \mathit{off}(a), \mathit{on}(b)}$ &  $S'_{30} = \set{ }$
\end{tabular}
\end{eqnarray*}
Now the lowest $\mathit{cost}_\mathit{noise}$ theory is one that finds the underlying regularity:
\begin{eqnarray*}
\begin{tabular}{lll}
$I = \bigsetbegin{}
\mathit{on}(a) \\
p_1(a) \\
p_2(b)
\bigsetend{}$ &
$R = \bigsetbegin{}
\mathit{off}(X) \rightarrow p_3(X) \\
p_2(X) \rightarrow \mathit{on}(X) \\
p_1(X) \fork \mathit{off}(X) \\
p_3(X) \fork p_2(X) \\
p_2(X) \fork p_1(X)
\bigsetend{}$ &
$C' = \bigsetbegin{}
\forall X {:}s, \; \mathit{on}(X) \oplus \mathit{off}(X) \\
\forall X {:}s, \; p_1(X) \oplus p_2(X) \oplus p_3(X)
\bigsetend{}$
\end{tabular}
\end{eqnarray*}
We can see, then, that the noise-robust version of the \sys{} is somewhat less data-efficient than the noise-intolerant version described earlier. 
\label{ex:noise-1}
\end{example}

\subsection{Experiments}

We used the following sequences to compare the noise-intolerant \sys{} with the noise-robust version:
\begin{center}
\begin{tabular}{ll}
\sequence{a,b,a,b,a,b,a,b,a,b,a,b} & \sequence{a,a,b,a,a,b,a,a,b,a,a,b} \\
\sequence{a,a,b,b,a,a,b,b,a,a,b,b} & \sequence{a,a,a,b,a,a,a,b,a,a,a,b} \\
\sequence{a,b,b,a,a,b,b,a,a,b,b,a} & \sequence{a,b,c,a,b,c,a,b,c,a,b,c} \\
\sequence{a,b,c,b,a,a,b,c,b,a,a,b,c,b,a} & \sequence{a,b,a,c,a,b,a,c,a,b,a,c} \\
\sequence{a,b,c,c,a,b,c,c,a,b,c,c} & \sequence{a,a,b,b,c,c,a,a,b,b,c,c}
\end{tabular}
\end{center}
We chose these particular sequences because they are simple, noise-free, and the \sys{} is able to solve them in a reasonably short time.

We performed two groups of experiments.
In the first, we evaluated how much longer the sequence needs to be for the noise-robust version to capture the underlying regularity, in comparison with the noise-intolerant version which is more data-efficient.
Figure \ref{fig:noise-1} shows the results. 
We plot mean percentage accuracy (over the ten sequences) against the length of the sequence that is provided to the \sys{}.
Note that the noise-intolerant version only needs sequences of length 10 to achieve 100\% accuracy, while the noise-tolerant version needs sequences of length 30.


\begin{figure}
  \centering
  \begin{tikzpicture}
    \begin{axis}[
        xmin=0,
        xmax=50,
        xtick={0,10,20,30,40, 50},
        ytick={0,0.25,0.5,0.75,1.0},
        ymin=0,
        ymax=1.0,
        xlabel={Length},
        ylabel={Accuracy},
        legend pos= south east
              ]
      \addplot coordinates{(2,0.4) (3, 0.3) (4, 0.4) (5, 0.3) (6, 0.5) (7, 0.6) (8, 0.9) (9, 1.0) (10, 1.0) (15, 1.0) (20, 1.0) (25, 1.0) (30, 1.0) (35, 1.0) (40, 1.0) (45, 1.0) (50, 1.0) } ;
      \addlegendentry{noise-intolerant}
      \addplot coordinates{(2, 0.4) (3, 0.3) (4, 0.2) (5, 0.3) (6, 0.3) (7, 0.5) (8, 0.3) (9, 0.3) (10, 0.3) (15, 0.5) (20, 0.7) (25, 0.9) (30, 0.9) (35, 1.0) (40, 0.9) (45, 1.0) (50, 1.0) };
      \addlegendentry{noise-robust}
    \end{axis}
  \end{tikzpicture}
\caption[Comparing the noise-robust and noise-intolerant versions for data-efficiency]{Comparing the data-efficiency of the noise-robust version of the \sys{} with the noise-intolerant version. We plot mean percentage accuracy against length of the sequence. The noise-intolerant version achieves 100\% accuracy when the sequence is length 10 or over, while the noise-robust version only achieves this level of accuracy when the length is over 30.}
\label{fig:noise-1}
\end{figure}


In the second experiment, we evaluate how much better the noise-robust version of the \sys{} is at handling mislabeled data.
We take the same ten sequences above, extended to length 100, and consider various perturbations of the sequence where we randomly mislabel a certain number of entries.
Figure \ref{fig:noise-2} shows the results.
We plot mean percentage accuracy (over the ten sequences) against the percentage of mislabellings. 
Note that the noise-intolerant version deteriorates to random as soon as any noise is introduced, while the noise-robust version is able to maintain reasonable accuracy with up to 30\% of the sequence mislabeled.

\begin{figure}
  \centering
  \begin{tikzpicture}
    \begin{axis}[
        xmin=0,
        xmax=50,
        xtick={0,10,20,30,40, 50},
        ytick={0,0.25,0.5,0.75,1.0},
        ymin=0,
        ymax=1.0,
        xlabel={Percentage of mislabelled data},
        ylabel={Accuracy},
        legend pos= south east
              ]
      \addplot coordinates{(0,1.0) (5, 0.4) (10, 0.4) (15, 0.4) (20, 0.4) (25, 0.4) (30, 0.4) (35, 0.4) (40, 0.4) (45, 0.4) (50, 0.4)  } ;
      \addlegendentry{noise-intolerant}
      \addplot coordinates{(0,1.0) (5, 0.96) (10, 0.92) (15, 0.96) (20, 0.97) (25, 0.96) (30, 0.88) (35, 0.76) (40, 0.56) (45, 0.52) (50, 0.51) };
      \addlegendentry{noise-robust}
    \end{axis}
  \end{tikzpicture}
\caption[Comparing the noise-robust and noise-intolerant versions for accuracy]{Comparing the accuracy of the noise-robust version of the \sys{} with the noise-intolerant version. We plot mean percentage accuracy against the number of mislabellings. The noise-intolerant version deteriorates to random as soon as any noise is introduced, while the noise-robust version is able to maintain reasonable (88\%) accuracy with up to 30\% of the sequence mislabelled.}
\label{fig:noise-2}
\end{figure}


==> tex/experiments.tex <==

\section{Experiments}
\label{sec:experiments}

\subsection{Five experimental domains}
\label{sec:domains}

To evaluate the generality of our system, we tested it in a variety of domains: elementary (one-dimensional) cellular automata,
drum rhythms and nursery tunes, sequence induction tasks, multi-modal binding tasks, and occlusion tasks.
These particular domains were chosen because they represent a diverse range of tasks that are simple for humans but are hard for state of the art machine learning systems.
The tasks were chosen to highlight the difference between mere perception (the classification tasks that machine learning systems already excel at) and apperception (assimilating information into a coherent integrated theory, something traditional machine learning systems are not designed to do).

\subsubsection{Results}
\label{sec:results-summary}

We implemented the \sys{} in Haskell and ASP.
We used \verb|clingo| \cite{gebser2014clingo} to solve the ASP programs generated by our system.
We ran all experiments with a time-limit of 4 hours.

Our experiments (on the prediction task) are summarised in Table \ref{table:experiments-overview}.
Note that our accuracy metric for a single task is rather exacting: the model is accurate (Boolean) on a task iff \emph{every} hidden sensor value is predicted correctly.\footnote{The reason for using this strict notion of accuracy is that, as the domains are deterministic and noise-free, there is a simplest possible theory that explains the sensory sequence. In such cases where there is a correct answer, we wanted to assess whether the system found that correct answer exactly -- not whether it was fortunate enough to come close while misunderstanding the underlying dynamics.} It does not score any points for predicting most of the hidden values correctly.
As can be seen from Table \ref{table:experiments-overview}, our system is able to achieve good accuracy across all five domains.

\begin{table}
\centering
\begin{tabular}{|l|p{1.2cm}|p{1.2cm}|p{1.7cm}|p{2.2cm}|p{1.5cm}|}
\hline
{\bf Domain} & {\bf Tasks (\#)} & {\bf Memory (megs)} & {\bf Input size (bits)} &  {\bf Held out size (bits)} & {\bf Accuracy (\%)} \\
\hline
ECA & 256 & 473.2 & 154.0 & 10.7 & 97.3\% \\
\hline
Rhythm \& music & 30 & 2172.5 & 214.4 & 15.3 & 73.3\% \\
\hline
\emph{Seek Whence} & 30 & 3767.7 & 28.4 & 2.5 & 76.7\% \\
\hline
Multi-modal binding & 20 & 1003.2 & 266.0 & 19.1 & 85.0\% \\
\hline
Occlusion & 20 & 604.3 & 109.2 & 10.1 & 90.0 \% \\
\hline
\end{tabular}
\caption[Results for prediction tasks on the five experimental domains]{Results for prediction tasks on five domains. We show the mean information size of the sensory input, to stress the scantiness of our sensory sequences. 
We also show the mean information size of the held-out data.
Our metric of accuracy for prediction tasks is whether the system predicted \emph{every} sensor's value correctly. }
\label{table:experiments-overview}
\end{table}

We briefly describe each of the five domains used for evaluation. 
For a full description of each domain, and our experimental methodology, see (TODO LINK).

\subsubsection{Elementary cellular automata}
\label{sec:eca}

An Elementary Cellular Automaton (ECA) \cite{wolfram1983statistical,cook2004universality} is a one-dimensional Cellular Automaton. 
The world is a circular array of cells. 
Each cell can be either $\mathit{on}$ or $\mathit{off}$.
The state of a cell depends only on its previous state and the previous state of its left and right neighbours.

\begin{figure}
\begin{center}
\begin{tikzpicture}[b/.style={draw, minimum size=3mm,   
       fill=black},w/.style={draw, minimum size=3mm},
       m/.style={matrix of nodes, column sep=1pt, row sep=1pt, draw, label=below:#1}, node distance=1pt]

\matrix (A) [m=0]{
|[b]|&|[b]|&|[b]|\\
&|[w]|\\
};
\matrix (B) [m=1, right=of A]{
|[b]|&|[b]|&|[w]|\\
&|[b]|\\
};
\matrix (C) [m=1, right=of B]{
|[b]|&|[w]|&|[b]|\\
&|[b]|\\
};
\matrix (D) [m=0, right=of C]{
|[b]|&|[w]|&|[w]|\\
&|[w]|\\
};
\matrix (E) [m=1, right=of D]{
|[w]|&|[b]|&|[b]|\\
&|[b]|\\
};
\matrix (F) [m=1, right=of E]{
|[w]|&|[b]|&|[w]|\\
&|[b]|\\
};
\matrix (G) [m=1, right=of F]{
|[w]|&|[w]|&|[b]|\\
&|[b]|\\
};
\matrix (H) [m=0, right=of G]{
|[w]|&|[w]|&|[w]|\\
&|[w]|\\
};
\end{tikzpicture}  
\caption[Updates for ECA rule 110]{Updates for ECA rule 110. The top row shows the context: the target cell together with its left and right neighbour. The bottom row shows the new value of the target cell given the context. A cell is black if it is on and white if it is off.}
\label{fig:update110}
\end{center}
\end{figure}
Figure \ref{fig:update110} shows one set of ECA update rules\footnote{This particular set of update rules is known as Rule $110$. Here, $110$ is the decimal representation of the binary $01101110$ update rule, as shown in Figure \ref{fig:update110}.  This rule has been shown to be Turing-complete \cite{cook2004universality}.}. 
Each update specifies the new value of a cell based on its previous left neighbour, its previous value, and its previous right neighbour. 
The top row shows the values of the left neighbour, previous value, and right neighbour.
The bottom row shows the new value of the cell.
There are 8 updates, one for each of the $2^3$ configurations.
In the diagram, the leftmost update states that if the left neighbour is $\mathit{on}$, and the cell is $\mathit{on}$, and its right neighbour is $\mathit{on}$, then at the next time-step, the cell will be turned $\mathit{off}$.
Given that each of the $2^3$ configurations can produce $\mathit{on}$ or $\mathit{off}$ at the next time-step, there are $2^{2^3} = 256$ total sets of update rules.

Given update rules for each of the 8 configurations, and an initial starting state, the trajectory of the ECA is determined.
Figure \ref{fig:trajectory110} shows the state sequence for Rule 110 above from one initial starting state of length 11.
\begin{figure}
\begin{center}
\begin{tikzpicture}[b/.style={draw, minimum size=3mm,   
       fill=black},w/.style={draw, minimum size=3mm},
       m/.style={matrix of nodes, column sep=1pt, row sep=1pt, draw, label=below:#1}, node distance=1pt]

\matrix (A) [m=110]{
|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
|[w]|&|[w]|&|[w]|&|[w]|&|[b]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
|[w]|&|[w]|&|[w]|&|[b]|&|[b]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
|[w]|&|[w]|&|[b]|&|[b]|&|[w]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
|[w]|&|[b]|&|[b]|&|[b]|&|[b]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
|[b]|&|[b]|&|[w]|&|[w]|&|[w]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
|[b]|&|[b]|&|[w]|&|[w]|&|[b]|&|[b]|&|[w]|&|[w]|&|[w]|&|[w]|&|[b]|\\
|[w]|&|[b]|&|[w]|&|[b]|&|[b]|&|[b]|&|[w]|&|[w]|&|[w]|&|[b]|&|[b]|\\
|[b]|&|[b]|&|[b]|&|[b]|&|[w]|&|[b]|&|[w]|&|[w]|&|[b]|&|[b]|&|[b]|\\
|[w]|&|[w]|&|[w]|&|[b]|&|[b]|&|[b]|&|[w]|&|[b]|&|[b]|&|[w]|&|[w]|\\
|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|&|[w]|\\
};
\node at (A-11-1) {?};
\node at (A-11-2) {?};
\node at (A-11-3) {?};
\node at (A-11-4) {?};
\node at (A-11-5) {?};
\node at (A-11-6) {?};
\node at (A-11-7) {?};
\node at (A-11-8) {?};
\node at (A-11-9) {?};
\node at (A-11-10) {?};
\node at (A-11-11) {?};
\end{tikzpicture}  
\end{center}
\caption[One trajectory for ECA rule 110]{One trajectory for Rule 110. Each row represents the state of the ECA at one time-step. In this prediction task, the bottom row (representing the final time-step) is held out. }
\label{fig:trajectory110}
\end{figure}

In our experiments, we attach sensors to each of the 11 cells, produce a sensory sequence, and then ask our system to find an interpretation that makes sense of the sequence.
For example, for the state sequence of Figure \ref{fig:trajectory110}, the sensory sequence is $(S_1, ..., S_{10})$ where:
\begin{eqnarray*}
S_1 & = & \set{\mathit{off}(c_1), \mathit{off}(c_2), \mathit{off}(c_3), \mathit{off}(c_4), \mathit{off}(c_5), \mathit{on}(c_6), \mathit{off}(c_7), \mathit{off}(c_8), \mathit{off}(c_(), \mathit{off}(c_{10}), \mathit{off}(c_{11})} \\
S_2 & = & \set{\mathit{off}(c_1), \mathit{off}(c_2), \mathit{off}(c_3), \mathit{off}(c_4), \mathit{on}(c_5), \mathit{on}(c_6), \mathit{off}(c_7), \mathit{off}(c_8), \mathit{off}(c_(), \mathit{off}(c_{10}), \mathit{off}(c_{11})} \\
S_3 & = & \set{\mathit{off}(c_1), \mathit{off}(c_2), \mathit{off}(c_3), \mathit{on}(c_4), \mathit{on}(c_5), \mathit{on}(c_6), \mathit{off}(c_7), \mathit{off}(c_8), \mathit{off}(c_(), \mathit{off}(c_{10}), \mathit{off}(c_{11})} \\
S_4 & = & \set{\mathit{off}(c_1), \mathit{off}(c_2), \mathit{on}(c_3), \mathit{on}(c_4), \mathit{off}(c_5), \mathit{on}(c_6), \mathit{off}(c_7), \mathit{off}(c_8), \mathit{off}(c_(), \mathit{off}(c_{10}), \mathit{off}(c_{11})} \\
S_5 & = & \set{\mathit{off}(c_1), \mathit{on}(c_2), \mathit{on}(c_3), \mathit{on}(c_4), \mathit{on}(c_5), \mathit{on}(c_6), \mathit{off}(c_7), \mathit{off}(c_8), \mathit{off}(c_(), \mathit{off}(c_{10}), \mathit{off}(c_{11})} \\
... &&
\end{eqnarray*}
Note that we do \emph{not} provide the spatial relation between cells. The system does not know that e.g.~cell $c_1$ is directly to the left of cell $c_2$. 

\paragraph{Results}
Given the 256 ECA rules, all with the same initial configuration, we treated the trajectories as a prediction task and applied our system to it.
Our system was able to predict 249 out of 256 correctly.
In each of the 7 out of 256 failure cases, the \sys{} found a unified interpretation, but this interpretation produced a prediction which was not the same as the oracle. 
In 242 out of 256 of the cases, our system produced a theory that exactly captures the dynamics of the ECA rules, a theory that predicts the ECA trajectories correctly no matter how many cells there are, or what initial configuration we start with.
For example, the dynamics found for Figure \ref{fig:trajectory110} above are:
\begin{eqnarray*}
R = \bigsetbegin{}
r(X, Y) \wedge \mathit{on}(X) \wedge \mathit{off}(Y) \fork \mathit{on}(Y) \\
r(X, Y) \wedge r(Y, Z) \wedge \mathit{on}(X) \wedge \mathit{on}(Z) \wedge \mathit{on}(Y) \fork \mathit{off}(Y)
\bigsetend{}
\end{eqnarray*}
These rules exactly capture the dynamics of the cells that \emph{change}. The other cells retain their value from the previous time-step, according to the frame axiom of Definition \ref{def:trace}.

The initial conditions found by the \sys{} describe the initial values of the cells, and also specify the latent $r$ relation between cells: 
\begin{eqnarray*}
I = \bigsetbegin{}
\begin{tabular}{lllllllllll}
$\mathit{off}(c_1)$ &
$\mathit{off}(c_2)$ &
$\mathit{off}(c_3)$ &
$\mathit{off}(c_4)$ &
$\mathit{off}(c_5)$ &
$\mathit{on}(c_6)$ &
$\mathit{off}(c_7)$ &
$\mathit{off}(c_8)$ &
$\mathit{off}(c_9)$ &
$\mathit{off}(c_{10})$ &
$\mathit{off}(c_{11})$ \\
$r(c_1, c_{11})$ &
$r(c_2, c_1)$ &
$r(c_3, c_2)$ &
$r(c_4, c_3)$ &
$r(c_5, c_4)$ &
$r(c_6, c_5)$ &
$r(c_7, c_6)$ &
$r(c_8, c_7)$ &
$r(c_9, c_8)$ &
$r(c_{10}, c_9)$ &
$r(c_{11}, c_{10})$
\end{tabular}
\bigsetend{}
\end{eqnarray*}
Here, the system uses $r(X, Y)$ to mean that cell $Y$ is immediately to the right of cell $X$.
Note that \emph{the system has constructed the spatial relation itself}. 
It was not given the spatial relation $r$ between cells.
All it was given was the sensor readings of the 11 cells.
It constructed the spatial relationship $r$ between the cells in order to make sense of the data.

\subsubsection{Drum rhythms and nursery tunes}
\label{sec:rhythms-and-tunes}

We also tested our system on simple auditory perception tasks.
Here, each sensor is an auditory receptor that is tuned to listen for a particular note or drum beat.
In the tune tasks, there is one sensor for $C$, one for $D$, one for $E$, all the way to $\mathit{HighC}$. (There are no flats or sharps).
In the rhythm tasks, there is one sensor listening out for bass drum, one for snare drum, and one for hi-hat.
Each sensor can distinguish four loudness levels, between 0 and 3. 
When a note is pressed, it starts at max loudness (3), and then decays down to 0.
Multiple notes can be pressed simultaneously. 

For example, the \emph{Twinkle Twinkle Little Star} tune generates the following sensor readings (assuming 8 time-steps for a bar):
\begin{eqnarray*}
S_1 & = & \set{ v(s_c, 3), v(s_d, 0), v(s_e, 0), v(s_f, 0),  v(s_g, 0), v(s_a, 0), v(s_b, 0), v(s_{c*}, 0) } \\
S_2 & = & \set{ v(s_c, 2), v(s_d, 0), v(s_e, 0), v(s_f, 0),  v(s_g, 0), v(s_a, 0), v(s_b, 0), v(s_{c*}, 0) } \\
S_3 & = & \set{ v(s_c, 3), v(s_d, 0), v(s_e, 0), v(s_f, 0),  v(s_g, 0), v(s_a, 0), v(s_b, 0), v(s_{c*}, 0) } \\
S_4 & = & \set{ v(s_c, 2), v(s_d, 0), v(s_e, 0), v(s_f, 0),  v(s_g, 0), v(s_a, 0), v(s_b, 0), v(s_{c*}, 0) } \\
S_5 & = & \set{ v(s_c, 1), v(s_d, 0), v(s_e, 0), v(s_f, 0),  v(s_g, 3), v(s_a, 0), v(s_b, 0), v(s_{c*}, 0) } \\
S_6 & = & \set{ v(s_c, 0), v(s_d, 0), v(s_e, 0), v(s_f, 0),  v(s_g, 2), v(s_a, 0), v(s_b, 0), v(s_{c*}, 0) } \\
...
\end{eqnarray*}

\paragraph{Results}
Recall that our accuracy metric is stringent and only counts a prediction as accurate if \emph{every} sensor's value is predicted correctly.
In the rhythm and music domain, this means the \sys{} must correctly predict the loudness value (between 0 and 3) for each of the sound sensors. There are 8 sensors for tunes and 3 sensors for rhythms. 
When we tested the \sys{} on the 20 drum rhythms and 10 nursery tunes, our system was able to predict 22/30 correctly.
Note that the interpretations found are large and complex programs by the standards of state of the art ILP systems.
In \emph{Three Blind Mice}, for example, the interpretation contained 10 update rules and 34 initialisation atoms making a total of 44 clauses.

\subsubsection{\emph{Seek Whence} and C-test sequence induction intelligent tests}
\label{sec:seek-whence}

Hofstadter introduced the \define{Seek Whence}\footnote{The name is a pun on ``sequence''. See also the related Copycat domain \cite{mitchell1993analogy}.} domain in \cite{hofstadter2008fluid}. 
The task is, given a sequence $s_1, ..., s_t$ of symbols, to predict the next symbol $s_{t+1}$.
%He began by considering traditional number sequences, sequences where extrapolating correctly required ``math savvy'': knowledge of certain peculiarly mathematical relations between numbers (e.g.~that $27$ can also be described as $3^3$). 
%But later he moved away from this domain-specific sequence extrapolation task, to a much more general domain-agnostic formulation.
%The ``Seek Whence'' domain is:
%\begin{quote}
%pattern-play involving small packets whose ingredients are smallish integers, and where the interrelationships between packets involve no mathematical notions beyond equality, successorship, and predecessorship \cite{hofstadter2008fluid}
%\end{quote}
Typical \emph{Seek Whence} tasks include\footnote{Hofstadter used natural numbers, but we transpose the sequences to letters, to bring them in line with the Thurstone letter completion problems \cite{thurstone1941factorial} and the C-test \cite{hernandez1998formal}.}:
\begin{itemize}
\item
\sequence{b, b, b, c, c, b, b, b, c, c, b, b, b, c, c}
\item
\sequence{a, f, b, f, f, c, f, f, f, d, f, f}
\item
\sequence{b, a, b, b, b, b, b, c, b, b, d, b, b, e, b}
\end{itemize}
Hofstadter called the third sequence the ``theme song'' of the \emph{Seek Whence} project because of its difficulty.
There is a ``perceptual mirage'' in the sequence because of the sub-sequence of five $b$'s in a row that makes it hard to see the intended pattern: $(b,x,b)^*$ for ascending $x$.

\begin{figure}
\centering
\begin{tabular}{|l|l|}
\hline
\sequence{a,a,b,a,b,c,a,b,c,d,a} & 
\sequence{a,b,c,d,e}\\
\sequence{b,a,b,b,b,b,b,c,b,b,d,b,b,e} &
\sequence{a,b,b,c,c,c,d,d,d,d,e}\\
\sequence{a,f,e,f,a,f,e,f,a,f,e,f,a} &
\sequence{b,a,b,b,b,c,b,d,b,e}\\
\sequence{a,b,b,c,c,d,d,e,e} &
\sequence{a,b,c,c,d,d,e,e,e,f,f,f}\\
\sequence{f,a,f,b,f,c,f,d,f} &
\sequence{a,f,e,e,f,a,a,f,e,e,f,a,a}\\
\sequence{b,b,b,c,c,b,b,b,c,c,b,b,b,c,c} &
\sequence{b,a,a,b,b,b,a,a,a,a,b,b,b,b,b}\\
\sequence{b,c,a,c,a,c,b,d,b,d,b,c,a,c,a} &
\sequence{a,b,b,c,c,d,d,e,e,f,f}\\
\sequence{a,a,b,a,b,c,a,b,c,d,a,b,c,d,e} &
\sequence{b,a,c,a,b,d,a,b,c,e,a,b,c,d,f}\\
\sequence{a,b,a,c,b,a,d,c,b,a,e,d,c,b} &
\sequence{c,b,a,b,c,b,a,b,c,b,a,b,c,b}\\
\sequence{a,a,a,b,b,c,e,f,f} &
\sequence{a,a,b,a,a,b,c,b,a,a,b,c,d,c,b}\\
\sequence{a,a,b,c,a,b,b,c,a,b,c,c,a,a,a} &
\sequence{a,b,a,b,a,b,a,b,a}\\
\sequence{a,c,b,d,c,e,d} &
\sequence{a,c,f,b,e,a,d}\\
\sequence{a,a,f,f,e,e,d,d} &
\sequence{a,a,a,b,b,b,c,c}\\
\sequence{a,a,b,b,f,a,b,b,e,a,b,b,d} &
\sequence{f,a,d,a,b,a,f,a,d,a,b,a}\\
\sequence{a,b,a,f,a,a,e,f,a} &
\sequence{b,a,f,b,a,e,b,a,d}\\
\hline
\end{tabular}
\caption{Sequences from \emph{Seek Whence} and the C-test}
\label{diag:sw}
\end{figure}

\paragraph{Results}
Given the 30 \emph{Seek Whence} sequences, we treated the trajectories as a prediction task and applied our system to it.
Our system was able to predict 23/30 correctly.
For the 7 failure cases, 4 of them were due to the system not being able to find any unified interpretation within the memory and time limits, while in 3 of them, the system found a unified interpretation that produced the ``incorrect'' prediction.

The first key point we want to emphasise here is that our system was able to achieve human-level performance\footnote{See Meredith \cite{meredith1986seek} for empirical results 25 students  on the``Blackburn dozen'' \emph{Seek Whence} problems.}  on these tasks without hand-coded domain-specific knowledge.\footnote{The one piece of domain-specific knowledge we inject is the successor relation between the letters $a$, $b$, $c$, ...}
This is a \emph{general} system for making sense of sensory data that, when applied to the \emph{Seek Whence} domain, is able to solve these particular problems.
%This is just what \cite{besold2015artificial,hernandez2016computer} argue is needed. 
The second point we want to stress is that our system did not learn to solve these sequence induction tasks after seeing many previous examples.\footnote{Machine learning approaches to these tasks need thousands of examples before they can learn to predict. See for example \cite{barrett2018measuring}.} 
On the contrary: our system had never seen any such sequences before; it confronts each sequence \emph{de novo}, without prior experience.
This system is, to the best of our knowledge, the first such general system that is able to achieve such a result.

\subsubsection{Binding tasks}
\label{sec:probe-task-binding}

The binding problem \cite{holcombe2009binding} is the task of recognising that information from different sensory modalities should be collected together as different aspects of a single external object.
For example, you hear a buzzing and a siren in your auditory field and you see an insect and an ambulance in your visual field.
How do you associate the buzzing and the insect-appearance as aspects of one object, and the siren and the ambulance appearance as aspects of a separate object?

To investigate how our system handles such binding problems,  we tested it on the following multi-modal variant of the ECA described above.
Here, there are two types of sensor. The light sensors have just two states: black and white, while the touch sensors have four states: fully un-pressed (0), fully pressed (3), and two intermediate states (1, 2).
After a touch sensor is fully pressed (3), it slowly depresses, going from states 2 to 1 to 0 over 3 time-steps.
In this example, we chose Rule 110 (the Turing-complete ECA rule) with the same initial configuration as in Figure \ref{fig:trajectory110}, as described earlier.
In this multi-modal variant, there are 11 light sensors, one for each cell in the ECA, and two touch sensors on cells 3 and 11.
See Figure \ref{fig:binding}.

\paragraph{Results} We ran 20 multi-modal binding experiments, with different ECA rules, different initial conditions, and the touch sensors attached to different cells. The engine achieved 85\% accuracy.


\begin{figure}
\begin{center}
\begin{tikzpicture}[b/.style={draw, minimum size=3mm,   
       fill=black},w/.style={draw, minimum size=3mm},
       m/.style={matrix of nodes, column sep=1pt, row sep=1pt, draw, label=below:#1}, node distance=1pt]

\matrix (A) [m=110]{
$l_1$&$l_2$&${\color{red}l_3}$&$l_4$&$l_5$&$l_6$&$l_7$&$l_8$&$l_9$&$l_{10}$&${\color{blue}l_{11}}$&$t_1$&$t_2$\\
W&W&{\color{red}W}&W&W&B&W&W&W&W&{\color{blue}W}&{\color{red}0}&{\color{blue}0}\\
W&W&{\color{red}W}&W&B&B&W&W&W&W&{\color{blue}W}&{\color{red}0}&{\color{blue}0}\\
W&W&{\color{red}W}&B&B&B&W&W&W&W&{\color{blue}W}&{\color{red}0}&{\color{blue}0}\\
W&W&{\color{red}B}&B&W&B&W&W&W&W&{\color{blue}W}&{\color{red}3}&{\color{blue}0}\\
W&B&{\color{red}B}&B&B&B&W&W&W&W&{\color{blue}W}&{\color{red}3}&{\color{blue}0}\\
B&B&{\color{red}W}&W&W&B&W&W&W&W&{\color{blue}W}&{\color{red}2}&{\color{blue}0}\\
B&B&{\color{red}W}&W&B&B&W&W&W&W&{\color{blue}B}&{\color{red}1}&{\color{blue}3}\\
W&B&{\color{red}W}&B&B&B&W&W&W&B&{\color{blue}B}&{\color{red}0}&{\color{blue}3}\\
B&B&{\color{red}B}&B&W&B&W&W&B&B&{\color{blue}B}&{\color{red}3}&{\color{blue}3}\\
W&W&{\color{red}W}&B&B&B&W&B&B&W&{\color{blue}W}&{\color{red}2}&{\color{blue}2}\\
?&?&?&?&?&?&?&?&?&?&?&?&?\\
};
\end{tikzpicture}  
\end{center}
\caption[A multi-modal trace of ECA rule 110 with light sensors and touch sensors]{A multi-modal trace of ECA rule 110 with eleven light sensors (left) $l_1, ..., l_{11}$ and two touch sensors (right) $t_1, t_2$ attached to cells 3 and 11. Each row represents the states of the sensors for one time-step. For this prediction task, the final time-step is held out.}
\label{fig:binding}
\end{figure}

\subsubsection{Occlusion tasks}
\label{sec:probe-task-binding}

Neural nets that predict future sensory data conditioned on past sensory data struggle to solve occlusion tasks because it is hard to inject into them the prior knowledge that objects persist over time.
Our system, by contrast, was designed to posit latent objects that persist over time.

To test our system's ability to solve occlusion problems, we generated a set of tasks of the following form:
there is a 2D grid of cells in which objects move horizontally.
Some move from left to right, while others move from right to left, with wrap around when they get to the edge of a row.
The objects move at different speeds. 
Each object is placed in its own row, so there is no possibility of collision.
There is an ``eye'' placed at the bottom of each column, looking up. 
Each eye can only see the objects in the column it is placed in.
An object is occluded if there is another object below it in the same column.
See Figure \ref{fig:occlusion}.


\begin{figure}
\centering
\includegraphics[scale=0.50]{figs/occlusion.pdf}
\caption{An occlusion task}
\label{fig:occlusion}
\end{figure}

The system receives a sensory sequence consisting of the positions of the moving objects whenever they are visible.
The positions of the objects when they are occluded is used as held-out test data to verify the predictions of the model.
This is an imputation task.

\paragraph{Results} 
We generated 20 occlusion tasks by varying the size of the grid, the number of moving objects, their direction and speed.
The \sys{} achieved 90\% accuracy.

\subsection{Empirical evaluations}
\label{sec:results}

In this section, we test our system to evaluate the truth of the following hypotheses:
\begin{enumerate}
\item
The five domains of section \ref{sec:domains} are challenging tasks for existing baselines.
\item
Our system handles retrodiction and imputation just as easily as prediction.
\item
The features of our system (unity conditions, cost minimisation) are essential to its performance.
\item
Our system outperforms state of the art inductive logic programming approaches in the five domains.
\end{enumerate}
We consider each in turn.

\subsubsection{The five domains of section \ref{sec:domains} are challenging tasks for existing baselines}
\label{sec:baselines}
To evaluate whether our domains are indeed sufficiently challenging, we compared our system against four baselines.
The first \define{constant} baseline always predicts the same constant value for every sensor for each time-step.
The second \define{inertia} baseline always predicts that the final hidden time-step equals the penultimate time-step. 
The third \define{MLP} baseline is a fully-connected multilayer perceptron (MLP) \cite{murphy2012machine} that looks at a window of earlier time-steps to predict the next time-step. 
The fourth \define{LSTM} baseline is a recurrent neural net based on the long short-term memory (LSTM) architecture \cite{hochreiter1997long}.

The neural baselines are designed to exploit potential statistical patterns that are indicative of hidden sensor states. In the MLP baseline, we formulate the problem as a multi-class classification problem, where the input consists in a feature representation ${\bf x}$ of relevant context sensors, and a feed-forward network is trained to predict the correct state ${\bf y}$ of a given sensor in question. In the prediction task, the feature representation comprises one-hot\footnote{A one-hot representation of feature $i$ of $n$ possible features is a vector of length $n$ in which all the elements are 0 except the $i$'th element.}  representations for the state of every sensor in the previous two time steps before the hidden sensor. The training data consists of the collection of all observed states in an episode (as potential hidden sensors), together with the respective history before. Samples with incomplete history window (at the beginning of the episode) are discarded.

The MLP classifier is a 2-layer feed-forward neural network, which is trained on all training examples derived from the current episode (thus no cross-episode transfer is possible). We restrict the number of hidden neurons to (20, 20) for the two layers, respectively, in order to prevent overfitting given the limited number of training points within an episode. We use a learning rate of $10^{-3}$ and train the model using the \emph{Adam} optimiser \cite{kingma2014adam} for up to $200$ epochs, holding aside 10\% of data for early stopping. 

Given that the input is a temporal sequence, a recurrent neural network (that was designed to model temporal dynamics) is a natural choice of baseline.
But we found that the LSTM performs only slightly better than the MLP on Seek Whence tasks, and worse on the other tasks. 
The reason for this is that the paucity of data (a single temporal sequence consisting of a small number of time-steps) does not provide enough information for the high capacity LSTM to learn desirable gating behaviour. The simpler and more constrained MLP with fewer weights is able to do slightly better on some of the tasks, yet both neural baselines achieve low accuracy in absolute terms.

Figure \ref{fig:baselines-chart} shows the results. Clearly, the tasks are very challenging for all four baseline systems.

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.25,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={predictive accuracy},
    symbolic x coords={eca,music,Seek-Whence},
    xtick=data,
    ]
\addplot[ybar, pattern=dots] coordinates {(eca,97) (music,73) (Seek-Whence,76)};
\addplot[ybar, pattern=north west lines] coordinates {(eca,8) (music,2) (Seek-Whence,26)};
\addplot[ybar, pattern=north east lines] coordinates {(eca,29) (music,0) (Seek-Whence,33)};
\addplot[ybar, pattern=grid] coordinates {(eca,14) (music,7) (Seek-Whence,17)};
\addplot[ybar, pattern=horizontal lines] coordinates {(eca,3) (music,0) (Seek-Whence,18)};
\legend{our system (AE),constant baseline, inertia baseline, MLP baseline, LSTM baseline}
\end{axis}
\end{tikzpicture}
\caption[Comparison with baselines]{Comparison with baselines. We display predictive accuracy on the held-out final time-step.}
\label{fig:baselines-chart}
\end{figure}

\subsubsection{Our system handles retrodiction and imputation just as easily as prediction}
\label{sec:retrodiction-imputation}

To evaluate whether our system is just as capable of retrodicting earlier values and imputing missing intermediate values as it is at predicting future values, we ran tests where the unseen hidden sensor values were at the first time step (in the case of retrodiction) or randomly scattered through the time-series (in the case of imputation).\footnote{A deterministic transition dynamic is a function from a set of ground atoms to a set of ground atoms. If this function is not injective, then information is lost as we go through time: there will be a unique next step from the current time-step, but there can be multiple previous steps that transition into the current time-step. Our search procedure uses maximum a posteriori (MAP) estimation: we find a single model with the highest posterior (based on the likelihood -- how well it explains the sequence, and on the prior -- the program length), and use that model to predict, retrodict, and impute. A more ambitious Bayesian approach would construct a probability distribution over rival theories, and use a mixture model for retrodiction. But, given the computation complexity of finding a single solution (see Section \ref{sec:complexity}),  this ambitious approach is -- in the short term at least -- prohibitively expensive.}
We made sure that the number of hidden sensor values was the same for prediction, retrodiction, and imputation.


\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.25,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={predictive accuracy},
    symbolic x coords={eca,music,Seek-Whence},
    xtick=data,
    ]
\addplot[ybar, pattern=dots] coordinates {(eca,97) (music,73) (Seek-Whence,76)};
\addplot[ybar, pattern=north east lines] coordinates {(eca,43) (music,70) (Seek-Whence,70)};
\addplot[ybar, pattern=grid] coordinates {(eca,89) (music,56) (Seek-Whence,80)};

\legend{prediction,retrodiction,imputation}
\end{axis}
\end{tikzpicture}
\caption[Comparing prediction with retrodiction and imputation]{Comparing prediction with retrodiction and imputation. In retrodiction, we display accuracy on the held-out initial time-step. In imputation, a random subset of atoms are held-out; the held-out atoms are scattered throughout the time-series. In other words, there may be different held-out atoms at different times. The number of held-out atoms in imputation matches the number of held-out atoms in prediction and retrodiction.}
\label{fig:retrodiction-and-imputation-chart}
\end{figure}

Figure \ref{fig:retrodiction-and-imputation-chart} shows the results.
The results are significantly lower for retrodiction in the ECA tasks, but otherwise comparable.
The reason for retrodiction's lower performance on ECA is that for a particular initial configuration there are a significant number (more than 50\%) of the ECA rules that wipe out all the information in the current state after the first state transition, and all subsequent states then remain the same. 
The results for imputation are comparable with the results for prediction. Although the results for rhythm and music are lower, the results on Seek Whence are slightly higher.

\subsubsection{The features of our system are essential to its performance.}
\label{sec:ablation}

To verify that the unity conditions are doing useful work, we performed a number of experiments in which the various conditions were removed, and compared the results.
We ran four ablation experiments.
In the first, we removed the check that the theory's trace covers the input sequence: $S \sqsubseteq \tau(\theta)$
(see Definition \ref{def:makes-sense}).
In the second, we removed the check on conceptual unity.
Removing this condition means that the unary predicates are no longer connected together via exclusion relations $\oplus$, and the binary predicates are no longer constrained by $\exists !$ conditions.
(See Definition \ref{def:conceptual-unity}).
In the third ablation test, we removed the check on spatial unity.
Removing this condition means allowing objects which are not connected via binary relations.
In the fourth ablation test, we removed the cost minimization part of the system.
%Recall from Section \ref{sec:system} that our system searches for the interpretation with the lowest cost (in our case, the size of the rules plus the number of initial conditions).
Removing this minimization means that the system will return the first interpretation it finds, irrespective of size.

The results of the ablation experiments are displayed in Table \ref{table:ablation}.
The first ablation test, where we remove the check that the generated sequence of sets of ground atoms respects the original sensory sequence ($S \sqsubseteq \tau(\theta)$), performs very poorly. 
Of course, if the generated sequence does not cover the given part of the sensory sequence, it is highly unlikely to accurately predict the held-out part of the sensory sequence. 
This test is just a sanity check that our evaluation scripts are working as intended.

The second ablation test, where we remove the check on conceptual unity, also performs poorly.
The reason is that without constraints, there are no incompossible atoms.
Recall from Definition \ref{def:trace} that two atoms are incompossible if there is some $\oplus$ constraint or some $\exists !$ constraint that means the two atoms cannot be simultaneously true.
%When there are no constraints, there are no incompossible atoms.
But in Definition \ref{def:trace}, the frame axiom forces an atom that was true at the previous time-step to also be true at the next time-step unless the old atom is incompossible with some new atom:
we add $\alpha$ to $H_t$ if $\alpha$ is in $H_{t-1}$ and there is no atom in $H_t$ that is incompossible with $\alpha$.
But if there are no incompossible atoms, then all previous atoms are always added.
Therefore, if there are no $\oplus$ and $\exists !$ constraints, then the set of true atoms monotonically increases over time.
This in turn means that state information becomes meaningless, as once something becomes true, it remains always true, and cannot be used to convey information. 

\begin{table}
\centering
\begin{tabular}{|l|r|r|r|}
\hline
& {\bf ECA} & {\bf Rhythm \& Music}  & {\bf Seek Whence} \\
\hline
Full system (AE) & 97.3\% & 73.3\% & 76.7\% \\
\hline
No check that $S \sqsubseteq \tau(\theta)$ & 5.1\% & 3.0\% & 4.6\% \\
\hline
No conceptual unity & 5.3\% & 0.0\% & 6.7\% \\
\hline
No spatial unity & 95.7\% & 73.3\% & 73.3\% \\
\hline
No cost minimization & 96.7\% & 56.6\% & 73.3\% \\
\hline
\end{tabular}
\caption[Ablation experiments]{Ablation experiments. We display predictive accuracy on the final held-out time-step.}
\label{table:ablation}
\end{table}

When we remove the spatial unity constraint, the results for the rhythm tasks are identical, but the results for the ECA and Seek Whence tasks are lower. 
The reason why the results are identical for the rhythm tasks is because the background knowledge provided (the $r$ relation on notes, see Section \ref{sec:rhythms-and-tunes}) means that the spatial unity constraint is guaranteed to be satisfied. 
The reason why the results are lower for ECA tasks is because interpretations that fail to satisfy spatial unity contain disconnected clusters of cells (e.g.~cells $\{c_1, ..., c_5\}$ are connected by $r$ in one cluster, while cells $\{c_6, ..., c_{11}\}$ are connected in another cluster, but  $\{c_1, ..., c_5\}$ and $\{c_6, ..., c_{11}\}$ are disconnected). Interpretations with disconnected clusters tend to generalize poorly and hence predict with less accuracy. 
The reason why the results are only slightly lower for the Seek Whence tasks is because the lowest cost unified interpretation for most of these tasks also happens to satisfy spatial unity. 

The results for the fourth ablation test, where we remove the cost minimization, are broadly comparable with the full system in ECA and Seek Whence, but are markedly worse in the rhythm / music tasks. 
But even if the results were comparable in all tasks, there are independent reasons to want to minimize the size of the interpretation. Shorter interpretations are more human-readable, and transfer better to new situations (since they tend to be more general, as they have fewer atoms in the bodies of the rules). 
%On the other hand, it is significantly more expensive to compute the lowest cost theory than it is to just find any unified theory (see the complexity results in Section \ref{sec:complexity}). So in some domains, where the difference in accuracy is minimal, the cost minimization step can be avoided. 

\subsubsection{Our system outperforms state of the art inductive logic programming approaches in the five domains}
\label{sec:ilasp}

In order to assess the efficiency of our system, we compared it to ILASP\footnote{We compared against ILASP rather than Metagol (another state of the art inductive logic programming system \cite{mugg:metagold,cropper}) because (i) ILASP is comparable in performance (it achieved slightly better results than Metagol in the Inductive General Game Playing task suite \cite{cropper2019inductive}, getting 40\% correct as opposed to Metagol's 36\%), and (ii) since ILASP also uses ASP we can compare the grounding size of our program with ILASP and get a fair apples-for-apples comparison. We used ILASP rather than HEXMIL (the ASP implementation of Metagol  \cite{kaminski2018exploiting}) because of scaling problems with HEXMIL \cite{cropper2019learning}. Our decision to use ILASP rather than Metagol for these tests was based on a number of discussions with Andrew Cropper (the developer of Metagol) and Mark Law (the developer of ILASP). We are very grateful to both for their advice on this.} \cite{law2014inductive,law2015learning,law2016iterative,law2018complexity}, a state of the art Inductive Logic Programming algorithm\footnote{Strictly speaking, ILASP is a family of 
algorithms, rather than a single algorithm. We used ILASP2 \cite{law2015learning} in this evaluation.}.
Unlike traditional ILP systems that learn definite logic programs, ILASP learns \emph{answer set programs}\footnote{Answer set programming under the stable model semantics is distinguished from traditional logic programming in that it is purely declarative and each program has multiple solutions (known as answer sets). Because of its non-monotonicity, ASP is well suited for knowledge representation and common-sense reasoning \cite{mueller2014commonsense,gelfond2014knowledge}.}.
ILASP is a powerful and general framework for learning answer set programs; it is able to learn choice rules, constraints, and even preferences over answer sets \cite{law2015learning}.

ILASP is able to solve some simple apperception tasks. For example, ILASP is able to solve the task in Example \ref{example:eca1}. 
But for the ECA tasks, the music and rhythm tasks, and the Seek Whence tasks, the ASP programs generated by ILASP were not solvable because they required too much memory.

In order to understand the memory requirements of ILASP on these tasks, and to compare our system with ILASP in a fair like-for-like manner, we looked at the size of the grounded ASP programs.
Recall that both our system and ILASP generate ASP programs that are then grounded into propositional clauses that are then passed to a SAT solver.
The grounding size determines the memory usage and is strongly correlated with solution time.

We took a sample ECA, Rule 245, and looked at the grounding size as the number of cells increased from 2 to 11.
The results are in Figure \ref{fig:grounding-comparison}.

\begin{figure}
\begin{center}
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={Number of cells in the ECA},
    ylabel={Grounding size (in megabytes)},
    xmin=2, xmax=11,
    ymin=0, ymax=7000,
    xtick={2,4,6,8,10},
    ytick={0,1000,2000,3000,4000,5000,6000,7000},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (2,60)(3,173)(4,376)(5,692)(6,1149)(7,1771)(8,2585)(9,3103)(10,4902)(11,6464)
    };
    \addlegendentry{ILASP}

\addplot[
    color=red,
    mark=*,
    ]
    coordinates {
    (2,1)(3,2)(4,4)(5,7)(6,13)(7,21)(8,31)(9,45)(10,61)(11,82)
    };
    \addlegendentry{Our system}
 
\end{axis}
\end{tikzpicture}
\end{center}
\caption{Comparing our system and ILASP w.r.t. grounding size}
\label{fig:grounding-comparison}
\end{figure}

As we increase the number of cells, the grounding size of the ILASP program grows much faster than the corresponding  \sys{} program. 
The reason for this marked difference is the different ways the two approaches represent rules.
In our system, rules are interpreted by an interpreter that operates on reified representations of rules.
In ILASP, by contrast, rules are \emph{compiled} into ASP rules.
This means, if there are $|U_\phi|$ unground atoms and there are at most $N_B$ atoms in the body of a rule, then ILASP will generate $|U_\phi|^{N_B+1}$ different clauses.
When it comes to grounding, if there are $|\Sigma_\phi|$ substitutions and $t$ time-steps, then ILASP will generate at most
$|U_\phi|^{N_B+1} \cdot |\Sigma_\phi| \cdot t$ ground instances of the generated clauses.
Each ground instance will contain $N_B + 1$ atoms, so there are $(N_B + 1) \cdot |U_\phi|^{N_B+1} \cdot |\Sigma_\phi| \cdot t$ ground atoms in total.

Compare this with our system. 
Here, we do not represent every possible rule explicitly as a separate clause.
Rather, we represent the possible atoms in the body of a rule by an ASP choice rule:
\begin{verbatim}
0 { rule_body(R, VA) : is_unground_atom(VA) } k_max_body :- is_rule(R).
\end{verbatim}
If there are $N_\rightarrow$ static rules and $N_{\fork}$ causal rules, then this choice rule only generates $N_\rightarrow + N_{\fork}$ ground clauses, each containing $|U_\phi|$ atoms. 

The most expensive clauses in our encoding are analysed in Table \ref{table:num-ground-clauses}.
Recall from Section \ref{sec:complexity} that the total number of atoms in the ground clauses is approximately $5 \cdot |\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot |U_\phi| \cdot t$. 

To compare this with ILASP, let us set $N_B = 4$ (which is representative). 
Then ILASP generates ground clauses with $5 \cdot |U_\phi|^{N_B+1} \cdot |\Sigma_\phi| \cdot t$ ground atoms while our system generates clauses with  $5 \cdot |\Sigma_\phi| \cdot (N_{\rightarrow} + N_{\fork}) \cdot |U_\phi| \cdot t$ ground atoms.

The reason, then, why our system has such lower grounding sizes than ILASP is because $(N_{\rightarrow} + N_{\fork})  << |U_\phi|^{N_B}$.
Intuitively, the key difference is that ILASP considers \emph{every possible} subset of the hypothesis space, while our system (by restricting to at most $N_{\rightarrow} + N_{\fork}$ rules) only considers \emph{subsets of length at most $N_{\rightarrow} + N_{\fork}$}.



==> tex/related-work.tex <==
\section{Related work}
\label{sec:discrete-related}

In this section, we describe particular systems that are related to our approach. For a general overview of the space of different approaches, see Section \ref{sec:intro-related}.

\subsection{``Theory learning as stochastic search in a language of thought''}
\label{sec:related-ullman}

Tomer Ullman et al \cite{goodman2011learning,ullman2012theory} describe a system for learning first-order rules from symbolic data.
Recasting their approach into our notation, their system is given as input a set $S$ of ground atoms\footnote{Compare with our system, which is given a sequence $(S_1, ..., S_T)$ of sets of ground atoms.}, and it searches for a set of static rules $R$ and a set $I$ of atoms such that $R, I \models S$.

Of course, the task as just formulated admits of entirely trivial solutions: for example, let $I = S$ and $R = \{\}$.
Ullman et al rule out such trivial solutions by adding two restrictions.
First, they distinguish between two disjoint sets of predicates:
the \emph{surface} predicates are the predicates that appear in the input $S$, while the \emph{core} predicates are the latent predicates. 
Only core predicates are allowed to appear in the initial conditions $I$.
This distinction rules out the trivial solution above, but there are other degenerate solutions:
for each surface predicate $p$, add a new core predicate $p_c$.
If $p(k_1, ..., k_n)$ is in $S$, add $p_c(k_1, ..., k_n)$ to $I$.
Also, add the rule $p(X_1, ..., X_n) \leftarrow p_c(X_1, .., X_n)$ to $R$.
Clearly, $R, I \models S$ but this solution is unilluminating, to say the least.
To prevent such degenerate solutions, the second restriction that Ullman et al add is to prefer \emph{shorter} rule-sets  $R$ and smaller sets $I$ of initial atoms.
The idea is that if $S$ contains structural regularities, their system will find an  $R$ and $I$ that are much simpler than the degenerate solution above.

Consider, for example, the various surface relations in a family tree: John is the father of William; William is the husband of Anne; Anne is the mother of Judith; John is the grandfather of Judith.
All the various surface relations (father, mother, husband, grandfather...) can be explained by a small number of core relations: $\mathit{parent}(X, Y)$, $\mathit{spouse}(X, Y)$, $\mathit{male}(X)$, and $\mathit{female}(X)$.
Now the surface facts $S = \{\mathit{father}(\mathit{john}, \mathit{william}), ...\}$ can be explained by a small number of facts involving core predicates $I = \{\mathit{parent}(\mathit{john}, \mathit{william}), \mathit{male}(\mathit{john}), ...\}$ together with rules such as:
\begin{eqnarray*}
\mathit{father}(X, Y) \leftarrow \mathit{parent}(X, Y), \mathit{male}(X)
\end{eqnarray*}

At the computational level, then, the task that Ullman et al set out to solve is: given a set $S$ of ground atoms featuring surface predicates, find the smallest set $I$ of ground atoms featuring only core predicates, and the smallest set $R$ of static rules, such that $R, I \models S$.
Recasting this task in the language of probability, they wish to find:
\begin{eqnarray*}
\operatorname*{arg\,max}_{R, I} p(R, I \mid S)
\end{eqnarray*}
Using Bayes' rule this can be recast as:
\begin{eqnarray*}
\operatorname*{arg\,max}_{R, I} p(R, I \mid S) & = & \operatorname*{arg\,max}_{R, I} \frac{p(S \mid R, I) p(R, I)}{p(S)} \\
& = & \operatorname*{arg\,max}_{R, I} p(S \mid R, I) p(R, I) \\
& = & \operatorname*{arg\,max}_{R, I} p(S \mid R, I) p(R) p(I \mid R)
\end{eqnarray*}
Here, the likelihood $p(S \mid R, I)$ is the proportion of $S$ that is entailed by $R$ and $I$, the prior $p(R)$ is the size of the rules, and $p(I \mid R)$ is the size of $I$.

At the algorithmic level, Ullman et al apply Markov Chain Monte Carlo (MCMC).
MCMC is a stochastic search procedure.
When it is currently considering search element $x$, it generates a candidate next element $x'$ by randomly perturbing $x$. 
Then it compares the scores of $x$ and $x'$.
If $x'$ is better, it switches attention to focus on $x'$. 
Otherwise, if $x'$ is worse than $x$, there is still a non-zero probability of switching (to avoid local minima), but the probability is lower when $x$' is significantly worse than the current search element $x$.

In their algorithm, MCMC is applied at two levels.
At the first level, a set $R$ of rules is perturbed into $R'$ by adding or removing atoms from clauses, or by switching one predicate for another predicate with the same arity. At the second level, $I$ is perturbed into $I'$ by changing the extension of the core predicates.

Given that the search space of sets of rules is so enormous, and that MCMC is a stochastic search procedure that only operates locally, the algorithm needs additional guidance to find solutions.
In their case, they provide a \emph{template}, a set of meta-rules that constrain the types of rules that are generated in the outermost MCMC loop. 
A meta-rule is a higher-order clause in which the predicates are themselves variables. 
For example, in the following meta-rule for transitivity, $P$ is a variable ranging over two-place predicates:
\begin{eqnarray*}
P(X, Y) \leftarrow P(X, Z), P(Z, Y)
\end{eqnarray*}
Meta-rules are a key component in many logic program synthesis systems \cite{mugg:metagold,crop:metafunc,crop:thesis,law2014inductive,law2018complexity}.

Ullman et al tested their system in a number of domains including taxonomy hierarchies, simplified magnetic theories, kinship relations, and psychological explanations of action. 
In each domain, their system is able to learn human-interpretable theories from small amounts of data.

At a high level, Ullman et al's system has much in common with the \sys{}.
They are both systems for generating interpretable explanations from small quantities of symbolic data.
While the \sys{} generates a $(\phi, I, R, C)$ tuple from a sequence $(S_1, ..., S_T)$, their system generates an $(I, R)$ pair from a single set $S$ of atoms.
But there are a number of significant differences.
First, our system takes as input a \emph{sequence} $(S_1, ..., S_T)$ while their system considers only a single state $S$.
Because they do not model facts changing over time, their system only needs to represent static rules and does not need to also represent causal rules.
Second, a unified interpretation $\theta = (\phi, I, R, C)$ in our system includes a set $C$ of \emph{constraints}.
These constraints play a critical role in our system: they are both regulative (ruling out certain incompossible combinations of atoms) and constitutive (the constraints determine the incompossible relation that in turn grounds the frame axiom). 
There is no equivalent of our constraints $C$ in their system.
A third key difference is that our system has to produce a theory that, as well as explaining the sensory sequence, also has to satisfy the \emph{unity conditions}: spatial unity, conceptual unity, static unity, and temporal unity.
There is no analog of our unity conditions in Ullman et al's system.
Fourth, their system requires \emph{hand-engineered templates} in order to find a theory that explains the input.
This reliance on hand-engineered templates restricts the domain of application of their technique:
in a domain in which they do not know, in advance, the structure of the rules they want to learn, their system will not be applicable.
Fifth, our system posits \emph{latent objects} as well as latent predicates, while their system only posits latent predicates.
The ability to imagine unobserved objects, with unobserved attributes that explain the observed attributes of observed objects, is a key feature of the \sys{}.

At the algorithmic level, the systems are very different.
While we use a form of meta-interpretive learning, they use MCMC.
Our system compiles an apperception problem into the task of finding an answer set to an ASP program that minimises the program cost. 
The ASP problem is given to an ASP solver, that is guaranteed to find the \emph{global minimum}.
MCMC, by contrast, is a stochastic procedure that operates \emph{locally} (moving from one single point in program space to another), and is not guaranteed to (in fact, in practice, it rarely does) find a global minimum. 

%Why use MCMC rather than a global method that is guaranteed to find a global minimum?
%One reason for using MCMC is if we want to construct a distribution over candidate theories, in order to generate predictions from a mixture model. If we have a way of predicting an element $x$ from a theory $\theta$, then we can predict $x$ from data $D$ by:
%\begin{eqnarray*}
%p(x \mid D) = \sum_{\theta} p(\theta \mid D) p(x \mid \theta)
%\end{eqnarray*}
%But this is not what Ullman et al actually do.
%Rather, they use MCMC to find a single point estimate, the maximum a posteriori (MAP) theory that best explains the data.
%Computing a distribution over theories is expensive in time and space. 
%As they acknowledge \cite{ullman2012theory}, humans typically only consider a tiny handful of rival theories, and often only just one. 
%
%One concern with MCMC approaches to program synthesis is that, typically, making one small change in a program requires many other changes to also be made, in order for that first change to be coherent. 
%Suppose $n$ changes are needed \emph{together} to make an improvement to a candidate rule set $R$.
%Since MCMC makes these $n$ changes \emph{individually},  and each of the first $n-1$ changes are on their own insufficient to gain an improvement over the initial $R$, the chances of MCMC making all $n$ changes and finding the improvement to $R$ is $k^{n-1}$ where $k$ is the mean change of making a suboptimal switch. 
%Since $k^{n-1}$ quickly tends to 0 as $n$ increases, the chances of MCMC finding large programs becomes increasingly small. 
%This is, we believe, the reason why the rule sets found by this approach are small (typically 2 to 4 clauses with at most 2 atoms in the body) in comparison with the programs found by the \sys{} (which can contain over 20 clauses with up to 5 atoms in the body). 

\subsection{``Learning from interpretation transition''}

Inoue, Ribeiro, and Sakama \cite{inoue2014learning} describe a system (\define{LFIT}) for learning logic programs from sequences of sets of ground atoms.
Since their task definition is broadly similar to ours, we focus on specific differences. 
In our formulation of the apperception task, we must construct a $(\phi, I, R, C)$ tuple from a sequence $(S_1, ..., S_T)$ of sets of ground atoms.
In their task formulation, they learn a set of causal rules from a set $\{(A_i, B_i)\}_{i=1}^N$ of pairs of sets of ground atoms.

In some respects, their task formulation is more general than ours.
First, their input  $\{(A_i, B_i)\}_{i=1}^N$ can represent transitions from \emph{multiple} trajectories, rather than just a single trajectory.
Second, they learn \emph{normal} logic programs, allowing negation as failure in the body of a rule, while our system only learns definite clauses. 

But there are a number of other ways in which our task formulation is significantly more general than LFIT. 
First, our system posits \emph{latent information} to explain the observed sequence, while LFIT does not construct any latent information. 
Their system searches for a program $P$ that generates \emph{exactly} the output state. In our approach, by contrast, we  search for a program whose trace \emph{covers} the output sequence, but does not need to be identical to it. The trace of a unified interpretation typically contains much extra information that is not part of the original input sequence, but that is used to explain the input information. 

Second, our system abduces a set of \emph{initial conditions} as well as a set of rules, while LFIT does not construct initial conditions. Because of this, our system is able to predict the future, retrodict the past, and impute missing intermediate values. 
LFIT, by contrast, can only be used to predict future values. 

Third, our system generates a set of \emph{constraints} as well as rules. The constraints perform double duty: on the one hand, they restrict the sets of compossible atoms that can appear in traces; on the other hand, they generate the incompossibility relation that grounds the frame axiom. Note that there is no frame axiom in LFIT.

In \cite{inoue2014learning}, Inoue et al use a bottom-up synthesis method to learn rules.
Given a state transition $(A, B)$ in $E$, they construct a normal ground rule for each $\beta \in B$:
\begin{eqnarray*}
\bigwedge_{\alpha \in A} \alpha \wedge \bigwedge_{\alpha \in \mathcal{G} - A} \mathit{not} \; \alpha \fork \beta
\end{eqnarray*}
Then, they use resolution to generalize the individual ground rules. 
It is important to note that this strategy is quite conservative in the generalizations it performs, 
since it only produces a more general rule if it turns out to be a resolvent of a pair of previous rules. 
While the \sys{} searches for the shortest (and hence most general) rules, LFIT searches for the most specific generalization.
In more recent work \cite{ribeiro2015learning}, LFIT has been changed to perform top-down specialization, rather than bottom-up generalization. With this change, LFIT is guaranteed to find the shortest set of rules that explain the transitions.  

LFIT was tested on Boolean networks and on Elementary Cellular Automata. 
It is instructive to compare our system with LFIT on the ECA tasks.
When LFIT is applied to the ECA task, it is provided with the one-dimensional spatial relation between the cells as background knowledge. 
In our approach, by contrast, we do \emph{not} hand-code the spatial relation, but rather let the \sys{} generate the spatial relation itself as part of the initial conditions. (See Section \ref{sec:eca}). It is precisely because our system is able to posit latent information to explain the surface features that it is able to generate the spatial relation itself, rather than having to be given it.

In some situations, positing latent information allow us to constructer a simpler theory.
In other situations, however, positing latent information is absolutely essential to making sense of the sequence: there are some apperception tasks for which every interpretation that makes sense of the sequence \emph{must} include latent information:
\begin{example}
Consider the task $(S, \phi, C)$ where $S = (S_1, S_2, S_3, ..., S_n)$, $S_1 = S_2= \{p(a)\}$, and $S_3 = S_4 = ... = S_n = \{q(a)\}$. Here, $\phi$ contains one type $t$, one object $a$ of type $t$, two unary predicates $p$ and $q$, and one constraint $\forall X: t, p(X) \oplus q(X)$. Since $p$ and $q$ are incompatible, the transition from $p$ to $q$ from state $S_2$ to $S_3$ must be explained by a causal rule $\phi \fork q(X)$, where $\phi$ is a set of atoms. Now $\phi$ cannot be empty, or the rule would be unsafe, $\phi$ cannot be $\{p(X)\}$, or else $q(a)$ would be derivable at the second time-step, contradicting $S_2 = \{p(a)\}$. Similarly, $\phi$ cannot be $\{q(X)\}$, or else $q(a)$ would not be derivable at time-step 3. Hence $\phi$ must contain an atom featuring a predicate distinct from $p$ or $q$. Hence, every interpretation that makes sense of $S$ must invoke latent information. 

One of the theories found by the \sys{} for this is $\theta = (\phi, I, R, C)$, where:
\begin{eqnarray*}
\begin{tabular}{lll}
$I = \bigsetbegin{}
p(a) \\
r(a)
\bigsetend{}$ &
$R = \bigsetbegin{}
r(X) \fork s(X) \\
p(X) \wedge s(X) \fork q(X)
\bigsetend{}$ &
$C = \bigsetbegin{}
\forall X {:}t, \; p(X) \oplus q(X) \\
\forall X {:}t, \; r(X) \oplus s(X)
\bigsetend{}$
\end{tabular}
\end{eqnarray*}
Here, there are two latent predicates, $r$ and $s$, that are used as counters, so the system can distinguish between the two occurrences of $p(a)$ in $S_1$ and $S_2$.
Thus for some sequences, the positing of latent predicates, and the abduction of initial conditions for the latent atoms, is \emph{unavoidable}.
\end{example}
LFIT has been extended in a number of ways, to increase the range of real-world problems that it can tackle.
In \cite{martinez2017relational}, LFIT was extended to learn probabilistic models.
In \cite{ribeiro2015learningb}, the system was extended from the Markov($1$) assumption (where the new state depends only on the current state) to the more general Markov($k$) setting (where the new state depends on the last $k$ states). 
In \cite{ribeiro2018learning}, LFIT was generalised so that as well as working with deterministic models (where all state transitions happen simultaneously), it also can work with other semantics (where only a subset of the transitions may happen at each time-step).
In \cite{ribeiro2017inductive}, LFIT was extended to work directly with continuous sensor data, rather than assuming the continuous sensor data has first been discretised by some other process. 
In \cite{tourret2017learning,phua2017learning}, LFIT was reimplemented in a feed-forward neural network, so as to robustly handle noisy and continuous data.

\subsection{``Unsupervised learning by program synthesis''}
\label{sec:related-ellis}

Kevin Ellis et al \cite{ellis2015unsupervised} use program synthesis to solve an unsupervised learning problem.
Given an unlabeled dataset $\{x_i\}_{i=1}^N$, they find a program $f$ and a set of inputs $\set{I_i}_{i=1}^N$ such that $f(I_i)$ is close to $x_i$ for each $i = 1 .. N$.
More precisely, they use Bayesian inference to find the $f$ and $\set{I_i}_{i=1}^N$ that minimizes the combined log lengths of the program, the initial conditions, and the data-reconstruction error:
\begin{eqnarray*}
-log P_f(f) + \sum_{i=1}^N \left( - log P_{x|z} (x_i \mid f(I_i)) - log P_I(I_i) \right)
\end{eqnarray*}
where $P_f(f)$ is a description length prior over programs, $P_I(I_i)$ is a description length prior over initial conditions, and $P_{x|z}(\cdot \mid z_i)$ is a noise model. 
This system was designed from the outset to be robust to noise, using Bayesian inference to calculate the desired tradeoff between the program length, the initial conditions length, and the data-reconstruction error cost.
They tested this system in two domains: reproducing two dimensional pictures, and learning morphological rules for English verbs.

This system is similar to ours in that it produces interpretable programs from a small number of data samples.
Like ours, their program length prior acts as an inductive bias that prefers general solutions over special-case memorized solutions.
Like ours, as well as constructing a program, they also learn initial conditions that combine with the program to produce the desired results.
At a high level, their algorithm is also similar: they generate a Sketch program \cite{solar2006combinatorial} from the dataset $\{x_i\}_{i=1}^N$ of examples, and use a SMT solver to fill in the holes.
They then extract a readable program from the SMT solution, which they then apply to new instances, exhibiting strong generalization.
Another point of similarity between this system and ours is that both systems struggle with large datasets. Because of the way problems are encoded and then compiled into SAT problems, the tasks get prohibitively large as the dataset increases in size. 

As well as the high level architectural similarities, there are a number of important differences.
First, their goal was to generate an object $f(I_i)$ that matches as closely as possible to the input object $x_i$. 
Our goal is more general: we seek to generate a sequence $\tau(\theta)$ that \emph{covers} the input sequence.
The covering relation is much more general, as $S_i$ only has to be a \emph{subset} of $(\tau(\theta))_i$, not identical to it.
This allows the addition of latent information to the trace of the theory.
A second key difference is that we focus on generating sequences, not individual objects. 
Our system is designed for making sense (unsupervisedly) of time series, sequences of states, not of reconstructing individual objects.
A third key difference is that we use a single domain-independent language, \logic{}, for all domains, while Ellis et al use a different domain-specific imperative language for each domain they consider.
A fourth key difference is that we use a declarative language, rather than an imperative language. 
An individual rule or constraint has a truth-conditional interpretation, and can be interpreted as a \emph{belief} of the synthesising agent. An individual line of an imperative procedure, by contrast, cannot be interpreted as a belief.
A fifth major difference is that we synthesise \emph{constraints} as well as rules.
Constraints are the ``special sauce'' of our system: exclusive disjunctions combine predicates into groups, enforce that each state is fully determinate, and ground the incompossibility relation that underlies the frame axiom. 

%\subsection[``Beyond imitation'']{``Beyond imitation: zero-shot task transfer on robots by learning concepts as cognitive programs''}
%\label{sec:related-vicarious}
%
%Miguel L\'azaro-Gredilla et al \cite{lazaro2018beyond} describe a system for learning procedural programs.
%Their system is given a set of input/output pairs (visual representations of the start state and target state), and learns a procedure that, when executed, transforms the input scene into the output scene.
%
%At a high level, this system is similar to ours in that it learns an interpretable program from a small number of examples.
%Like our system, they have a program length prior that prefers small general programs to large special-case programs, so their learned programs tend to generalize well to new situations.
%Their system shares the same underlying assumption as ours: concepts are programs in a language of thought, learned from sensory input. 
%
%However, there are a number of key differences between our approaches.
%First, our system operates on time series with a built-in domain-independent understanding of persistence (see the frame axiom in Definition \ref{def:trace}). 
%While they operate in a static world (the ``tabletop world'') where the only agent that initiates change is the self, our system attempts to make sense of a dynamic world where any object can initiate changes.   
%Second, they concentrate on supervised program synthesis using input/output pairs, while we focus on \emph{unsupervised} program synthesis. 
%Third, we use a declarative language for describing concepts, while they use an imperative one.
%For them, a concept is a procedure to change the world in a certain way (e.g.~``stack green objects on the right'').
%For us, a concept is a predicate that can appear in a declarative sentence.
%Fourth, our system includes constraints as well as update rules. These xor and uniqueness constraints are the key distinctive aspect of our architecture: they allow concepts to be unified into groups, they provide determinacy in the states of the trace, and they ground the incompossibility relation that underlies the frame axiom. 
%Finally, their system has a very distinctive architecture that combines visual attention, imagination, a vision hierarchy, and a dynamics model. 
%We respect their unapologetic use of architectural bias, but note that their architecture is very different from ours. 

\subsection{``Learning symbolic models of stochastic domains''}
\label{sec:related-learning-symbolic-models}

Hanna Pasula et al \cite{pasula2007learning} describe a system for learning a state transition model from data.
The model learns a probability distribution $p(s' \mid s, a)$ where $s$ is the previous state, $a$ is the action that was performed and $s'$ is the next state. 

Each state is represented as a set of ground atoms, just like in our system.
They assume \emph{complete observability}: they assume they are given the value of every sensor and the task is just to predict the next values of the sensors.

They represent a state transition model by a set of ``dynamic rules'': these are first-order clauses determining the future state given a current state and an action. These dynamic rules are very close to the causal rules in \logic{}. Unlike in our system, their rules have a probability outcome for each possible head. %This extends work by Benson \cite{benson1996learning}. 
Note their system does not include static rules or constraints.

In their semantics, they assume that \emph{exactly one dynamic rule fires every tick}. This is a very strong assumption. But it makes it easier to learn rules with probabilistic outcomes. 

They learn state transitions for the noisy gripper domain (where a robot hand is stacking bricks, and sometimes fails to pick up what it attempts to pick up) and a logistics problem (involving trucks transporting objects from one location to another). Impressively, they are able to learn probabilistic rules in noisy settings.
They also verify the usefulness of their learned models by passing them to a planner (a sparse sampling MDP planner), and show, reassuringly, that the agent achieves more reward with a more accurate model.

At a strategic level, their system is similar in approach to ours.
First, they learn first-order rules, not merely propositional ones. In fact, they show in ablation studies that learning propositional rules generalises significantly less well, as you would expect.
Second, they use an inductive bias against constants (p.14), just as we do: ``learning action models which are restricted to be free of constants provides a useful bias that can improve generalisation when training with small data sets''. 
Third, their system is able to construct new invented predicates. 

But there are also a number of differences. 
In our system, many rules can fire simultaneously. 
But in theirs, only one rule can fire in any state. 
Because of this assumption, they cannnot model e.g.~a cellular automaton, where each cell has its own individual update rule firing simultaneously.
Another limiting assumption is that they assume they have complete observability of all sensory predicates. 
This means they would not be able to solve e.g.~occlusion tasks.  
%More generally, they assume that a subset of events has been distinguished as exogenous actions and that only actions can create state changes. In our more general system, events bring about other events. In the \sys{}, we are not given complete $(s, a, s')$ triples for supervised learning, but sequences of partial information $(S_1, S_2, ...)$.

\subsection{``Nonmonotonic abductive inductive learning''}
\label{sec:related-work-xhail}

Oliver Ray \cite{ray2009nonmonotonic} described a system, \define{XHAIL}, for jointly learning to abduce ground atoms and induce first-order rules. 
XHAIL learns normal logic programs that can include negation as failure in the body of a rule. 

XHAIL is similar to the \sys{} in that as well as inducing general first-order rules, it also constructs a set of initial ground atoms. 
This enables it to model latent (unobserved) information, which is a very powerful and useful feature.
At the implementation level, it uses a similar strategy in that solutions are found by iterative deepening over a series of increasingly complex ASP programs.
The simplified event calculus \cite{kowalski1989logic} is represented explicitly as background knowledge.

But there are also a number of key differences.
First, it does not model constraints. This means it is not able to represent the incompossibility relation between ground atoms. 
Also, XHAIL does not try to satisfy our other unity conditions, such as spatial and conceptual unity.
Second, the induced rules are \emph{compiled} in XHAIL, rather than being interpreted (as in our system). 
Representing each candidate induced rule explicitly as a separate ASP rule means that the number of ASP rules considered grows exponentially with the size of the rule body\footnote{It shares the same implementation strategy as ASPAL \cite{corapi2012inductive} and ILASP \cite{law2014inductive}. See Section \ref{sec:ilasp} for discussion of the grounding problem associated with this family of approaches. The discussion is specifically focused on ILASP, but we believe the same issue affects ASPAL and XHAIL \emph{mutatis mutandem}.}.
Third, XHAIL needs to be provided with a set of mode declarations to limit the search space of possible induced rules.
These mode declarations constitute a significant piece of background knowledge.
Now of course there is nothing wrong with allowing an ILP system to take advantage of background knowledge to aid the search. But when an ILP system \emph{relies} on this hand-engineered knowledge, then it restricts the range of applicability to domains in which human engineers can anticipate in advance the form of the rules they want the system to learn\footnote{See Appendix C of \cite{evans2018learning} for a discussion of the use of mode declarations as a language bias in ILP systems.}.

\subsection{The Game Description Language and inductive general game playing}
\label{sec:distinctive-aspects}

Our language \logic{} is an extension of Datalog that incorporates, as well as the standard static rules of Datalog, both causal rules (Definition \ref{def:rules}) and constraints (Definition \ref{def:constraints}). 
The semantics of \logic{} are defined according to Definition \ref{def:trace}.
Unlike standard Datalog, the atoms and rules of \logic{} are strongly typed.

At a high level, \logic{} is related to the Game Description Language (GDL) \cite{love2008general}.
The GDL is an extension of Datalog that was designed to express deterministic multi-agent discrete Markov decision processes. 
The GDL includes (stratified) negation by failure, as well as some (restricted) use of function symbols, but these extensions were carefully designed to preserve the key Datalog property that a program has a unique subset-minimal Herbrand model.
The GDL includes special keywords, including \verb|init| for specifying initial conditions (equivalent to the initial conditions $I$ in a $(\phi, I, R, C)$ theory), and \verb|next| for specifying state transitions (equivalent to our causal rules). 
The \emph{inductive general game playing} (IGGP) task \cite{genesereth2013international,cropper2019inductive} involves learning the rules of a game from observing traces of play. 

An IGGP task is broadly similar to an apperception task in that both involve inducing initial conditions and rules from traces. 
But there are many key differences. 
One major feature of \logic{} is the use of \emph{constraints} to generate incompossible sets of ground atoms.
These exclusion constraints are needed to generate the incompossibility relation which in turn is needed to restrict the scope of the frame axiom (see Definition \ref{def:trace}). 

The main difference between \logic{} and the GDL is that the former includes exclusion constraints.
The exclusion constraints play two essential roles.
First, they enable the theory as a whole to satisfy the condition of conceptual unity.
Second, they provide constraints, via the condition of static unity, on the generated trace: since the constraints must always be satisfied, this restricts the rules that can be constructed.
Satisfying these constraints means \emph{filling in missing information}. 
This is why a unified interpretation is able to make sense of incomplete traces where some of the sensory data is missing. 


\subsection{Other related work}
\label{sec:other-related-work}

We briefly outline four other related topics.
One related area of research is learning action theories \cite{moyle2002using,otero2005induction,inoue2005inducing,corapi2011probabilistic,rodrigues2011active}. 
Here, the aim is to learn the transition dynamics in the presence of exogenous actions performed by an agent.
The aim is not to predict what actions the agent performs, but rather to predict the effects of the action on the state. 

A second related area is relational reinforcement learning \cite{dvzeroski2001relational,de2008logical,bu2008comprehensive}.
Here, the agent works out how to optimize its reward in an environment by constructing (using ILP) a first-order model of the dynamics of that environment, which it then uses to plan. 

A third related area is learning game rules from player traces \cite{goodacre1996inductive,law2014inductive}.
Here, the learning system is presented with traces (typically, sequences of sets of ground atoms), representing the state of the game at various points in time, and has to learn the transition dynamics (or reward function, or action legality function) of the underlying system. 

A fourth related area is the predictive processing (PP) paradigm \cite{friston2005theory,friston2012history,clark2013whatever,swanson2016predictive}, an increasingly popular model in computational and cognitive neuroscience.
Inspired by Helmholtz (who was in turn inspired by Kant \cite{swanson2016predictive}), the model learns to make sense of its sensory stream by attempting to predict future percepts. When the predicted percepts diverge from the actual percepts, the model updates its parameters to minimize prediction error. The PP model is probabilistic, Bayesian, and hierarchical: probabilistic in that the predicted sensory readings are represented as probability density functions, Bayesian in that the likelihood (represented by the information size of the misclassified predictions) is combined with prior expectations \cite{friston2012history}, and hierarchical in that each layer provides predictions of sensory input for the layer below; there are typically many layers.
One key difference between our approach and PP is that while PP focuses on prediction, the \sys{} generates an interpretation that is equally adept at predicting future signals, retrodicting past signals, and imputing missing intermediary signals. 
In our approach, the ability to predict future signals is a derived capacity, a capacity that emerges from the more general capacity to construct a unified interpretation -- but prediction is not singled out in particular. The \sys{} is able to predict, retrodict, and impute -- in fact, it is able to do all three \emph{simultaneously} using a single incomplete sensory sequence with elements missing at the beginning, at the end, and in the middle.

%Another key difference is how the two approaches address Hume's problem of induction: the problem, roughly, of justifying causal statements on the basis of scanty and particular instances of associations. 
%While Hume attempted to solve the problem by asserting that humans do, as a matter of contingent empirical fact, have a tendency to posit causal relations, Kant claimed that agents \emph{must} posit causal relations in order to perceive temporal succession. In Kant's solution, necessity is required at two levels: first, we must (deontic necessity) posit causal laws in order to perceive succession; second, the law itself states what must (alethic necessity) happen when its antecedent is satisfied. 
%
%PP uses probabilistic Bayesian inference to conclude that certain sensory percepts are highly probable given other sensory percepts.
%For Kant, by contrast, causal rules do not apply to \emph{most} instances with a certain probability; rather, they apply to \emph{all} of the instances with the ``dignity of necessity''.
%We claim that the \sys{}, which posits universally quantified necessary causal rules in order to generate temporal succession, is closer to Kant's understanding of causation than PP.
%
%A third key difference between our approach and PP is that our approach insists on conceptual unity, which can only be achieved by positing xor constraints which combine predicates into clusters. There is no equivalent of conceptual unity via constraints in PP approaches so far.





